MatRox: Modular approach for improving data locality in Hierarchical (Mat)rix App(Rox)imation

Hierarchical matrix approximations have gained significant traction in the machine learning and scientific community as they exploit available low-rank structures in kernel methods to compress the kernel matrix. The resulting compressed matrix, HMatrix, is used to reduce the computational complexity of operations such as HMatrix-matrix multiplications with tuneable accuracy in an evaluation phase. Existing implementations of HMatrix evaluations do not preserve locality and often lead to unbalanced parallel execution with high synchronization. Also, current solutions require the compression phase to re-execute if the kernel method or the required accuracy change. In this work, we describe MatRox, a framework that uses novel structure analysis strategies, blocking and coarsen, with code specialization and a storage format to improve locality and create load-balanced parallel tasks for HMatrix-matrix multiplications. Modularization of the matrix compression phase enables the reuse of computations when there are changes to the input accuracy and the kernel function. The MatRox-generated code for matrix-matrix multiplication is 2.98x, 1.60x, and 5.98x faster than library implementations available in GOFMM, SMASH, and STRUMPACK respectively. Additionally, the ability to reuse portions of the compression computation for changes to the accuracy leads to up to 2.64x improvement with MatRox over five changes to accuracy using GOFMM.

==> Figures/MatRoxRUrun.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}


    \begin{lstlisting}[frame=none, mathescape=true]
#include <matrox.h>
#include "mul_gen.h"
int main(){
    // Loading inputs to MatRox-RU
   Points points("path/to/point/directory");
   float tau = 1.4;
   Sampling sam_info("path/to/sampling/info");
   StructureSet block("path/to/block/set");
   Tree clsuter_tree("path/to/cluster/tree");
   Ktype kfunc = KS_GAUSSIAN;

   // Tuning for accuracy using MatRox-RU
   for(acc in {1e-3, 1e-4, 1e-5}){
       HMatrix H = MatRox_RU(points, tau,sam_info,block,cluster_tree, kfunc, acc);
        // Mul_gen is generated by MatRox
       y = Mul_gen(H,w);
       // Compute the error norm
    }
    return 0;
}
    
      \end{lstlisting}

==> Figures/block.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}
\definecolor{rs1}{rgb}{0,0.8,1}
\definecolor{rs2}{rgb}{0.67,0.67,0.83}
\definecolor{rs3}{rgb}{0.4,0.7,1}
\definecolor{rs4}{rgb}{0.7,0.8,1}
\definecolor{rs5}{rgb}{0.8,0.8,0.9}
\definecolor{rs6}{rgb}{0.47,0.47,0.7}

\lstset{
	%columns=fullflexible,
	keywords=[2]{Coarsen, Block, peel, vec},
	keywords=[3]{pass},
	keywordstyle={\color{blue!80!black}},
	keywordstyle=[2]{\color{rs6}},
	keywordstyle=[3]{\color{green!50!black}},
}
\begin{lstlisting}[frame=none, mathescape=true,
otherkeywords={Coarsen, Block,...}]
#pragma omp parallel for
for(every block $k$ in nblockset ){
	for(every $v$ $\in$ nblockset[$k$]){
		$i$ = $v[0]$; $j$ = $v[1]$;
		|\textcolor{grayLine}{	$\textrm{y}_{i}$ = $\textrm{D}_{{i,j}}$ * ${\textrm{w}}_{j}$; }|
}}
\end{lstlisting}

==> Figures/coarsen.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}


	\begin{lstlisting}[frame=none, mathescape=true]
for($cl$ in coarsenset){| \label{line:bcl}|
#pragma omp parallel for
   for($st$ in $cl$-partition) { |\label{line:pLoop}  |     
	    for($i$ in $st$-subtree ){ |\label{line:ecl}|
		    |\textcolor{grayLine}{if(i is leaf node)}|
			    |\textcolor{grayLine}{$\textrm{tw}_i$ = $\textrm{V}_i^T$ * $\textrm{w}_i$;}|
		    |\textcolor{grayLine}{else }|
	      |\textcolor{grayLine}{// use results from children }|
          |\textcolor{grayLine}{$lc$ = lchild(i); $rc$ = rchild[i]; }|
          |\textcolor{grayLine}{$\textrm{tw}_i$ = $\textrm{V}_i^T$  * $\textrm{tw}_{lc}$; }|
          |\textcolor{grayLine}{	$\textrm{tw}_i$ = $\textrm{V}_i^T$  * $\textrm{tw}_{rc}$; }|
	    }
    }
}
	
	  \end{lstlisting}

==> Figures/codestyle.tex <==
\definecolor{commentgreen}{RGB}{2,112,10}
\definecolor{grayLine}{RGB}{100,100,100}
\definecolor{annotation}{rgb}{0.45, 0.31, 0.59}
\definecolor{darklavender}{rgb}{0.45, 0.31, 0.59}
\lstset{ %
language=C++,                % choose the language of the code
basicstyle=\ttfamily\footnotesize,       % the size of the fonts that are used for the code
columns=fullflexible,
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                 % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
%backgroundcolor=\color{codeBG3},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
commentstyle=\color{commentgreen}\ttfamily,
escapeinside={\%*}{*)},          % if you want to add a comment within your code
keywordstyle=\color{blue},       % keyword style
  %language=Octave,                 % the language of the code
  otherkeywords={SearchVar,MV,TSS,tileExpr,Search,std::string, Ktype, HMatrix, Dense, HGEMM, OP, Points, Tree, StructureSet, Sampling, tFunc...},           % if you want to add more keywords to the set
  numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},
  escapechar=|
}

==> Figures/codestyle1.tex <==
\definecolor{commentgreen}{RGB}{2,112,10}
\definecolor{grayLine}{RGB}{100,100,100}
\definecolor{annotation}{rgb}{0.45, 0.31, 0.59}
\definecolor{darklavender}{rgb}{0.45, 0.31, 0.59}
\lstset{ %
language=C++,                % choose the language of the code
basicstyle=\ttfamily\footnotesize,       % the size of the fonts that are used for the code
columns=fullflexible,
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                 % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
%backgroundcolor=\color{codeBG3},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
commentstyle=\color{commentgreen}\ttfamily,
escapeinside={\%*}{*)},          % if you want to add a comment within your code
keywordstyle=\color{blue},       % keyword style
  %language=Octave,                 % the language of the code
  otherkeywords={SearchVar,MV,TSS,tileExpr,Search,std::string, Ktype, HMatrix, Dense, HGEMM, OP, Points, StructureSet, Sampling, tFunc...},           % if you want to add more keywords to the set
  numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},
  escapechar=|
}

==> Figures/fmmblock-v1.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}
	\begin{lstlisting}[frame=none, mathescape=true]
//near interactions
for(every block $k$ in nblockset ){
	for(every $v$ $\in$ nblockset[$k$]){
		$i$ = $v[0]$; $j$ = $v[1]$;
		$\textrm{y}_{i}$ = $\textrm{D}_{{i,j}}$ * ${\textrm{w}}_{j}$;}}
|\textcolor{grayLine}{$\textrm{tw}$ = ${V}^T$ * $\textrm{w}$ }|
//far ineractions
for(every block $k$ in fblockset){
  for(every $v$ $\in$ fblockset[$k$]){
		$i$ = $v[0]$; $j$ = $v[1]$;
		$\textrm{tu}_{i}$ = $\textrm{B}_{i,j}$ * $\textrm{tw}_{j}$; }}
|\textcolor{grayLine}{$\textrm{y}$ += $\textrm{tu}$ * $U$ }|
	  \end{lstlisting}

==> Figures/hssblock-v1.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}
	\begin{lstlisting}[frame=none, mathescape=true]
//near interactions
for(every leaf node $i$){
  $j$ = $i$;
	$\textrm{y}_{i}$ = $\textrm{D}_{{i,j}}$ * ${\textrm{w}}_{j}$;
}
|\textcolor{grayLine}{$\textrm{tw}$ = ${V}^T$ * $\textrm{w}$ }|
//far ineractions
for(every node $i$){
	$j$ = $i \& 1?:i+1,i-1$;
	$\textrm{tu}_{i}$ = $\textrm{B}_{i,j}$ * $\textrm{tw}_{j}$; 
}
|\textcolor{grayLine}{$\textrm{y}$ += $\textrm{tu}$ * $U$ }|
	  \end{lstlisting}

==> Figures/inputcode.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}


	\begin{lstlisting}[frame=none, mathescape=true]
int main(int argc, char const *argv[]){
    	Points points("path/to/point/directory");
    	//type of kernel function
    	Ktype kfunc=KS_GAUSSIAN;
    	//class for Hierarchical matrices
    	HMatrix K(Float(64), points, tau, kfun, acc);
	    Dense W(Float(64), nrhs);
	    Dense Y(Float(64));
    	OP Mul(K, W, Y);
    	//class for code generation
    	Mul.generate_to_c("../../CodeGen/mul_gen");
	    return 0;
}
	
	  \end{lstlisting}

==> Figures/level.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}
\definecolor{rs1}{rgb}{0,0.8,1}
\definecolor{rs2}{rgb}{0.67,0.67,0.83}
\definecolor{rs3}{rgb}{0.4,0.7,1}
\definecolor{rs4}{rgb}{0.7,0.8,1}
\definecolor{rs5}{rgb}{0.8,0.8,0.9}
\definecolor{rs6}{rgb}{0.47,0.47,0.7}

\lstset{
	%columns=fullflexible,
	keywords=[2]{Coarsen, Block, peel, vec},
	keywords=[3]{pass},
	keywordstyle={\color{blue!80!black}},
	keywordstyle=[2]{\color{rs6}},
	keywordstyle=[3]{\color{green!50!black}},
}
\begin{lstlisting}[frame=none, mathescape=true,
otherkeywords={Coarsen, Block,...}]
Coarsen: for($l$ in Tree.height..1){
   for(every node i $\in$ level l) { |\label{line:pLoop}|
     |\textcolor{grayLine}{if(i is leaf node)}|
			 |\textcolor{grayLine}{$\textrm{tw}_i$ = $\textrm{V}_i^T$ * $\textrm{w}_i$;}|
		 |\textcolor{grayLine}{else }|
	   |\textcolor{grayLine}{// use results from children }|
       |\textcolor{grayLine}{$lc$ = lchild(i); $rc$ = rchild[i]; }|
       |\textcolor{grayLine}{$\textrm{tw}_i$ = $\textrm{V}_i^T$  * $\textrm{tw}_{lc}$; }|
       |\textcolor{grayLine}{	$\textrm{tw}_i$ = $\textrm{V}_i^T$  * $\textrm{tw}_{rc}$; }|
    }
}
\end{lstlisting}

==> Figures/matroxrun.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}


    \begin{lstlisting}[frame=none, mathescape=true]
#include <matrox.h>
#include "mul_gen.h"
int main(int argc, char const *argv[]){
        HMatrix H = load_cds("/path/to/cds");
        double W = random(H.n, nrhs);
        double Y = new double[H.n*nrhs];
        Y = Mul_gen(H,W);
        //process Y
        return 0;
}
    
      \end{lstlisting}

==> Figures/nonblock.tex <==
\newcommand{\cL}{{\cal L}}
\input{Figures/codestyle.tex}
\definecolor{rs1}{rgb}{0,0.8,1}
\definecolor{rs2}{rgb}{0.67,0.67,0.83}
\definecolor{rs3}{rgb}{0.4,0.7,1}
\definecolor{rs4}{rgb}{0.7,0.8,1}
\definecolor{rs5}{rgb}{0.8,0.8,0.9}
\definecolor{rs6}{rgb}{0.47,0.47,0.7}

\lstset{
	%columns=fullflexible,
	keywords=[2]{Coarsen, Block, peel, vec},
	keywords=[3]{pass},
	keywordstyle={\color{blue!80!black}},
	keywordstyle=[2]{\color{rs6}},
	keywordstyle=[3]{\color{green!50!black}},
}
\begin{lstlisting}[frame=none, mathescape=true,
otherkeywords={Coarsen, Block,...}]
Block: for(every leaf node $i$){
	for(every node $j \in$ near[i]){
	  |\textcolor{grayLine}{	$\textrm{y}_{i}$ = $\textrm{D}_{{i,j}}$ * ${\textrm{w}}_{j}$; }|
    }
}
\end{lstlisting}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> SRC/Extra.tex <==
 \section{MatRox-RU: Re-Using inspector with changes to input}\label{sec:matroxrc}

% \begin{tabular}{ |c|c|c| } 
%  \hline
%   & Compile-time & Run-time \\ 
%  \hline
%  Solution A & tree construction, compute interaction, sampling, structure analysis, compression w/o sampling,  code generation  &   evaluation \\ 
%  \hline
%  Solution B & tree construction, compute interaction, sampling, structure analysis, code generation  & compression w/o sampling, binpacking, data layout construction, evaluation   \\ 
%  \hline
% \end{tabular}
% Given points and kernel function, the structure of kernel matrix can be reasoned according to the distribution of points and kernel function.
% The approximation error depends on the points and kernel function.

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.8\columnwidth]{Figures/matrox-cr.jpg}
%     \caption{MatRox compression at runtime}
%     \label{fig:my_label}
% \end{figure*}


\begin{figure}
    \centering
    \input{Figures/matroxru_in.tex}
    \caption{MatRox-RU: Re-Using inspector with changes to input}
    \label{fig:my_label}
\end{figure}

%In several real applications, user only changes kernel function or accuracy requirements. For example for finding a trade-off between accuracy and performance, one needs to run both structure analysis and evaluation phases several times and with different accuracy requirements until the expected performance and accuracy is achieved.   
 %Also, in some application it happens often that property of the kernel function changes. For example, in kernel-based learning method, Gaussian kernel parameterized by a bandwidth $h$ is commonly used and cross-validation is leveraged to select h. That requires approximation for kernel matrix generated using Gaussian kernel with different values of $h$.

%Kernel matrices and semi positive definite (SPD) matrices in general, appear in  machine learning, scientific computing and data analytics. For example, they appear in solving linear system equations using Cholesky factorization\cite{grasedyck2008parallel}, saddle point problems in computational science such as finite elements\cite{benzi2005numerical}, Hessian methods for nonlinear optimizations\cite{muske2000lagrangian} and statistical learning such as support vector machines (SVM)\cite{hofmann2008kernel}. In all these applications, the matrix representing the system does not change throughout the iterative computations. For example, in finite element methods (FEM), the stiffness matrix is used in a linear system of equations with only right hand side changing throughout the computations. Similarly, in statistical learning problems such as SVM , the kernel matrix is constructed using a invariable(?can't find a better word) training dataset and a kernel function. Therefore, the training dataset or the points which the kernel matrix is generated from remains the same through the specified underlying algorithm. 

%in FEM points are actually the mesh, n-body points dont move alot [], machines these are features ** and you train on sepcfici ***. 
%At this point, there are only some loose upper bounds on the accuracy of the kernel matrix that relate to the block accuracy[ASKIT].
%For example, in kernel-based learning method, Gaussian kernel parameterized by a bandwidth $h$ is commonly used and cross-validation is leveraged to select h. That requires approximation for kernel matrix generated using Gaussian kernel with different values of $h$. 

%The underlying algorithms in these applications aim to solve a linear systems of equations using an iterative approach for a given kernel matrix and a right hand side (e.g. the stiffness matrix and source function in FEM)\cite{grasedyck2008parallel}. If the kernel matrix is approximated using a H-matrix, the solution of the linear system is also approximated. Currently, there are no works that connect the accuracy of the solution of the linear system to the accuracy of the kernel matrix approximation. Moreover, the kernel matrix is approximated using hierarchical approach in which sub-matrices of the kernel matrix are approximated to satisfy a block accuracy (e.g., $b-acc$ in MatRox). At this point, there are only some loose upper bounds on the accuracy of the kernel matrix that relate to the block accuracy[ASKIT]. Therefore, it is crucial to tune the block accuracy through trial and errors to meet the desired accuracy of the output of the specified iterative algorithm. 





In several real applications, user only changes kernel function or accuracy requirements.  While the input points typically don't change in applications, e.g.  the same dataset is used throughout a machine learning application and in scientific simulations changes to the points are typically slow [],  the input accuracy and the kernel function parameters often might change during a simulation.  In many scientific and machine learning applications the practitioner needs to change the input accuracy (bacc) because (1) the overall accuracy of the HMatrix-matrix multiplication is not sufficient. The input bacc is used to control the accuracy with which the low rank blocks in $K$ are approximated, however, depending on the dataset and the [FIXME: say something about Eigenvalue spectrum and low rankness]  this might not be the same as the overall accuracy of evaluation. Thus the users often need to re-compress the matrix for a more accuracy evaluation; (2) HMatrix evaluations are used to trade of accuracy for performance, i.e. matrix multiplication with a more compressed matrix is typically faster but less accurate. Thus, the domain expert might want to re-compress the matrix to do faster evaluation with less accuracy. Also,  in some application the parameters  of the kernel function are tuned during simulation. For example, in kernel-based learning method, the Gaussian kernel parameterized by a bandwidth $h$ is commonly used with cross-validation  to select h. 
 
The modular design in MatRox, allows for the reuse of specific components of the inspector when parts of the input change. In libraries any change to the inputs requires running the entire compression and evaluation phase. However, when the kernel function and/or the input accuracy change in MatRox, the modules and components in the inspector that do not rely on these inputs and the components involved can execute only once and be reused. MatRox-RU enables this reuse by separating the inspector into two phases, i.e. inspector-p1 and inspector-p2. A change in the kernel function and/or the accuracy only requires inspector-p2 and the executor to be reran. Figure shows MatRox-RU's flow and an example code that allows for the reuse of inspector-P1 when the bacc changes. 


%Because of its modular design, the 


%Matrox supports running the three mentioned blocks i.e., low-rank approximation, coarsening, and data layout construction in in a sperate isnepction phase which we call inspector-p2 in figure **. This will allow the the reuse of output of other blocks such as interaction information, the cluster tree, sampling information, and block set.  We refer this solution in MatRox as MatRox-CR (MatRox compression at run-time). In addition to reusing these components, MatRox also reuses some information within  \autoref{alg:partAlg}. As discusses in \autoref{sec:sa}, the tree coarsening has three steps that only its last step, i.e., binpacking has to be changed after change in the rank information. MatRox-CR also reuses the information from the first two steps and only re-run the binpacking stage shown in lines~\ref{line:bpack}-\ref{line:epack} of \autoref{alg:partAlg}.   



%MatRox-CR can provide several benefits by reusing structure information over library or normal MatRox's solution. 
%Firstly,  when the set of input points do not change,  tree construction and sampling is only done once and always be reused for low rank approximation. This reuse reduces the overhead of compression for high dimension points significantly, in which sampling is much more expensive than low rank approximation.  
%Secondly, it reduces I/O overhead led by writing and reading CDS from disk. In MatRox-RU, we only need to save and read cluster tree from disk. 
%Thirdly, the more runs in tuning accuracy or selecting kernel functions, the more performance benefits are achieved through using MatRox-CR.


%As shown by Figure \ref{fig:structure},  the whole structure analysis phase is at compile-time to generate structure-specific code. Using this scenario, changing any input parameters, e.g., kernel function or accuracy requirements requires re-compilation since the structure varies with all inputs. MatRox is designed to be able reuse information for these scenarios.

%MatRox decomposes the structural analysis phase into different fine-grain components that allows reusing information for some realistic scenarios. As shown in \autoref{fig:structure}, changing accuracy requirement and/or kernel function only requires recomputing low-rank approximation, coarsening, and data layout construction components. 





% In Figure \ref{fig:structure}, the structure analysis components corresponding to rank information include low-rank approximation, coarsening and data layout construction. As the main part of compression phase, low-rank approximation is moved to run-time and generates the rank information.
% Tree coarsening algorithm requires rank information to estimate the computation cost shown in line \ref{line:bcost}-\ref{line:ecost} of Algorithm \ref{alg:partAlg} and merge disjoint subtrees using binpack algorithm shown in line \ref{line:bpack}-\ref{line:epack} of Algorithm \ref{alg:partAlg}. Therefore, cost estimation and binpack parts are also moved to run-time to generate the coarsen-set at run-time. 
% The data layout construction can also be done at run-time after tree coarsening is completed. 

% Depending on interaction information, blocking transformation can be done without knowing ranks.
% While only part of tree coarsening algorithm is executed to find disjoint subtrees at compile-time, the coarsening transformation can still be leveraged to generate the code iterating over coarsen-set. 
% Therefore, blocking and coarsening transformation will not be affected by the lack of rank information. 
% Low-level transformations such as peeling for loop to use parallel BLAS will also not be affected since it is based on tree information.  

% The compression phase can be moved to runtime which enables the reuse of structure for cases where accuracy and the kernel function change frequently.
% The reason behind that is the input accuracy requirement just reflects the error of the subsampled blocks in the compression phase and may not control the resulting error of computation in the evaluation phase directly. There is no rule of thumb about setting parameters to satisfy a prescribed tolerance in one-shot. 
% Therefore, it relies on user to tune the parameters like accuracy requirement to satisfy accuracy requirement. On another hand, the property of kernel function changes sometimes. For example, in kernel-based learning method, Gaussian kernel parameterized by a bandwidth $h$ is commonly used and cross-validation is leveraged to select h. That requires approximation for kernel matrix generated using Gaussian kernel with different values of $h$. 


% Since changing the input accuracy requirement or kernel functions only corresponds to rank information, MatRox-CR exploits tree and interaction information to build structure set at compile-time to generate structure-specific code. All the computations related to rank information part shown in Figure \ref{fig:structure} will be done at run-time: 1) low rank approximation; 2) binpack part in tree coarsening part, which requires rank information to estimate the computation cost; 3) data layout construction. 
% Blocking transformation is not affected since it is based on interaction information. Coarsening transformation is also not affected since the number of partitions in each level will be known in advance based on cluster tree. Therefore, the low-level transformations related to cluster tree and interaction will not be affected. 
% Without rank information, the low-level transformations such as using specific BLAS routines can not be done. 





\subsection{The Performance of MatRox-RU}



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/acc.eps}
    \caption{Relative error on all matrices, tested on FMM [FIXME:bacc]}
    \label{fig:acc}
\end{figure}

In Figure \ref{fig:acc}, we show the correlation between input $b-acc$ and relative accuracy $\epsilon_f$. There are two reasons why user may require to tune accuracy. 
As shown in Figure \ref{fig:acc} in some benchmarks such as covtype, susy and unit to reach accuracy $1e-3$, user needs to tune $2$ times average even with the assumption that initially user gives the input $b-acc=1e-3$ and hopes to reach the accuracy.  
For some detasets there is a good correlation between input accuracy and output accuracy, for example, sunflower dataset returns $9e-5$ given the input accuracy $b-acc=1e-3$ without tuning. 
In other scenarios, often the user would require a low accurate result that could run the code faster, which means they would require to change the input accuracy.  
This is why tuning accuracy is important and MatRox-RU presents a more efficient way of tuning the accuracy by reusing part of inspector. In Figure \ref{fig:matnrun}, we show average 5 times of tuning input accuracy , which is typical number of times that input would be tuned in applications. 
It is important to know that some datasets do not reach the desired accuracy like mnist.
[FIXME: We need to add bacc=-10 and this sentences has ot be corrected] The matrix generated from mnist doesn't have good hierarchical low-rank structure and requires more effective clustering to partition points in extremely high dimensional space, which will be added to MatRox in future. 


We demonstrate the performance benefits provided by MatRox-RU in this subsection. 
Figure \ref{fig:matnrun} shows the end to end time comparison between MatRox and GOFMM, in which we set input accuracy $b-acc$ to 1e-1, 1e-2, 1e-3, 1e-4 and 1e-5 for 5 runs to show the effect of reusing part of inpsection at compile-time. 
In real case, the user may need to tune more than 5 runs to obtain faster code or more accurate result since the $b-acc$ is block approximated may not correspond to the result accuracy. We take GOFMM and SMASH as two reference tools for evaluating performance of MatRox-RU. 

% 1) GOFMM is the fastest existing libraries for FMM on shared memory environment; 2) MatRox and GOFMM are based on same compression algorithm and the effect of reusing inspector can be shown clearly. 


As shown in Figure \ref{fig:matnrun}, MatRox enables partial reuse of inspection (MatRox inspection P1) . 
For the overall performance, MatRox-RU's inspection plus execution time is on average  $2.21\times$ faster than GOFMM code after 5 runs due to partial reuse of inspection and faster evaluation code. 
Sampling takes more time for high dimensional points because the computation complexity of sampling is proportial to dimension of points. 
For high dimension points such as covtype and mnist, MatRox is on average $2.30\times$ and $2.64\times$ faster than GOFMM code because sampling takes $51.0\%$ and $89.2\%$ of the compression time and reusing it can lead to significant performance improvement.  
The overall execution time of MatRox-RU is on average $1.37\times$ faster than SMASH. For two dimensional points such as sunflower and unit, MatRox-RU is slower than SMASH due to SMASH's fast compression phase. 



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/matnruns.eps}
    \caption{Multiple runs for FMM on Haswell.}
    \label{fig:matnrun}
\end{figure}


\begin{table}
%\begin{small}
\begin{tabular}{|c|ccc|cc|}
	\hline
\multirow{2}{*}{Dataset}	& \multicolumn{3}{c}{MatRox} & \multicolumn{2}{c|}{SMASH} \\
	\cline{2-6}
	& P1& P2 & eval & comp & eval \\
	\hline
grid &  0.97  & 1.8  & 0.14 & 4.32 & 0.22 \\
random &  0.29 & 0.9 & 0.09 & 1.23 & 0.14 \\
dino &  0.58 & 3.05 & 1.10 & 9.84 & 1.52 \\
sunflower & 0.42 & 1.30  &   0.11 & 1.57 & 0.16 \\
unit &  0.26 & 0.50 &  0.10 & 0.62 &  0.17 \\
\hline

\end{tabular}
%\end{small}
\caption{Multiple runs for H2 on Haswell. P1 denotes inspector P1 phase, P2 denots inspector P2 phase. [FIXME: Add a speedup column]}
\end{table}


% For 
% The inspection in MatRox performs $1.36\times$ faster over GOFMM's compression phase due to reuse. MatRox-RU can bring more performance benefits for high dimensional points. For example, the inspection in MatRox is $2.87\times$ faster than GOFMM's compression phase for mnist dataset with 780 dimension, because sampling takes $89.1\%$ of the time of GOFMM's compression phase and MatRox can provide significant performance improvement by reusing sampling information. 




% \subsection{Overhead of generating CDS in MatRox}
% ??

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/hssa.eps}
%     \includegraphics[width=\columnwidth]{Figures/knlhssa.eps}
%     \caption{
%     Normalized execution time relative to MatRox for HSS approximation on Haswell (top) and Bottom (bottom). Missing bar denotes that the datasets cannot be processed by that library.
%     % The figure shows the compile and run time for MatRox, and run-time for GOFMM library for HSS-structure matrices on Haswell (top) and KNL(bottom). All times are normalized over GOFMM's run time. (lower is better. ) Kernel function is Gaussian with bandwidth  $5$ and number of right hand sides is 2048. Input accuracy requirement is $1e-5$. 
%     % Using budget=$0\%$ from GOFMM to enforce HSS approximation. Other parameters are kept as same as GOFMM's default parameters.
%     }
%     \label{fig:hss-sa}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/fmma.eps}
%     \includegraphics[width=\columnwidth]{Figures/knlfmma.eps}
%     \caption{
%      Normalized execution time relative to MatRox for FMM approximation on Haswell (top) and Bottom (bottom). Missing bar denotes that the datasets cannot be processed by that library.
%     % The figure shows the compile and run time for MatRox, and run-time for GOFMM library for FMM-structure matrices on Haswell (top) and KNL (bottom). All times are normalized over GOFMM's run time. (lower is better. ) kernel function is Gaussian with bandwidth  $5$ and number of right hand sides is 2048.  Input accuracy requirement is $1e-5$.
%     % Using budget=$3\%$ from GOFMM to enforce FMM approximation. Other parameters are kept as same as GOFMM's default parameters.
%     }
%     \label{fig:fmm-sa}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/strumpacksa.eps}
    
%     \caption{The figure shows the compile and run time for MatRox, and run-time for STRUMPACK library for HSS-structure matrices. All times are normalized over STRUMPACK's run time. (lower is better. ) Kernel function is Gaussian with bandwidth  $5$ and number of right hand sides is 2048. 
%     Input accuracy requirement is $1e-5$.
%     Set admissibility condition $\tau=10$ to enforce HSS approximation. Other parameters are kept as same as STRUMPACK's default parameters.}
%     \label{fig:strumpack-sa}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/smash.eps}
%     \caption{
%     The figure shows the upperbound of MatRox's speedup over SMASH for H2-structure matrices. All times are normalized over SMASH's run time. (higher is better. ) Kernel function is newton.
%   Input accuracy requirement is $1e-5$.
%     using admissbility condition $\tau=0.65$ from SMASH. Other parameters are kept as same as SMASH's default parameters.
%     }
%     \label{fig:smash-sa}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/hssnruns.eps}
%     \includegraphics[width=\columnwidth]{Figures/fmmnruns.eps}
%     \caption{multiple runs by tuning input accuracy requirement from 1e-1 to 1e-5  in 5 runs for HSS(top) and FMM(bottom)}
%     \label{fig:my_label}
% \end{figure}



% \begin{figure}
%     \centering
   
%     \caption{Scalability result on KNL. Test Dataset: covtype (left) and unit (right).}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.45\columnwidth]{Figures/scalcovtype.eps}
%     \includegraphics[width=0.45\columnwidth]{Figures/scalunit.eps}
%     \includegraphics[width=0.45\columnwidth]{Figures/knlscal.eps}
%     \includegraphics[width=0.45\columnwidth]{Figures/knlscalunithss.eps}
%     \caption{Scalability result for HSS}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.45\columnwidth]{Figures/fmmscal1.eps}
%     \includegraphics[width=0.45\columnwidth]{Figures/fmmscal2.eps}
%     \includegraphics[width=0.45\columnwidth]{Figures/knlfmmscal.eps}
%     \includegraphics[width=0.45\columnwidth]{Figures/knlfmmscalunit.eps}
%     \caption{Scalability result for FMM}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\columnwidth]{Figures/h2scal1.eps}
%     \includegraphics[width=0.45\columnwidth]{Figures/h2scalunit.eps}
%     \caption{Scalability result for H2}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/hssnrunsh.eps}
%     \includegraphics[width=\columnwidth]{Figures/fmmnrunsh.eps}
%     \caption{Changing kernel function}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/fmmnruns.eps}
%     \includegraphics[width=\columnwidth]{Figures/knlfmmnruns.eps}
%     \caption{multiple runs by tuning input accuracy requirement from 1e-1 to 1e-5  in 5 runs for FMM-structure matrices on Haswell(top) and KNL(bottom)}
%     \label{fig:my_label}
% \end{figure}




% \begin{figure*}
%     \centering
%     \includegraphics[width=1.8\columnwidth]{Figures/hss-separate.eps}
%     \caption{MatRox's generated code for evaluation phase compared to GOFMM for HSS-structure matrix. The stacked-bars shows MatRox code with coarsening transformation. 
%     The effects of CDS and coarsening transformations on MatRox perform are shown separately. 
%     configuration: budget is 0.0 to enforce HSS approximation, input accuracy requirement is 1e-5, kernel function is Gaussian with bandwidth is $5$ and number of right hand sides is 2048. Other parameters are kept same as GOFMM to give a fair comparison.
% %Here we use Here we use GOFMM's method (budget) provided by GOFMM instead of $\tau$ in admissibility condition to determine near and far interactions. Budget=$0\%$ means to enfore all off-diagonal blocks will be approximated. 
%     }
%     \label{fig:hssresults}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.8\columnwidth]{Figures/fmm-separate.eps}
%     \caption{MatRox's generated code for evaluation phase compared to GOFMM for FMM-structure matrix.
%      The stacked-bars shows MatRox code with blocking and coarsening transformation. 
%     The effects of CDS and coarsening transformations on MatRox  are shown separately. 
%     configuration: budget is $3\%$ to enforce FMM approximation, input block accuracy is 1e-5 in MatRox?, kernel function is Gaussian with bandwidth  $5$ and number of right hand sides is 1024. Other parameters are kept same as GOFMM to give a fair comparison. 
%     %Here we use Here we use GOFMM's method (budget) provided by GOFMM instead of $\tau$ in admissibility condition to determine near and far interactions. Budget=$3\%$ means to enforce $3\%$ off-diagonal blocks will not be approximated. 
%     }
%     \label{fig:fmmresults}
% \end{figure*}
















% The compression phase can be moved to runtime which eliminates the enables the reuse of structure for cases where accuracy and the kernel function change. One of the structure information which is the rank has to be determined only at runtime which also requires us to move the binpacking to runtime. Figure ** shows the different between theses approaches. 


% \begin{figure*}
%     \centering
%     \begin{tabular}{c|c}
        
%         \subfloat[Solution A]{
%         \includegraphics[width=0.95\columnwidth]{Figures/solutiona-v1.pdf}
%         }
%          &  
%          \subfloat[Solution B]{
%          \includegraphics[width=\columnwidth]{Figures/solutionb-v1.pdf}
%          }
%          \\
         
%     \end{tabular}
%     \caption{Solution A vs Solution B}
%     \label{fig:solab}
% \end{figure*}



\section{MatRox: Code Generation with Structure Analysis for Matrix Approximations }
MatRox is a framework that analyzes  structure at compile-time in  hierarchical matrix approximations   to generate efficient code and data layout for H-Matrix evaluations. Example input code to MatRox is shown in Listing ** in which the user provides the points, the kernel function, the admissibility condition, block accuracy, and the evaluation operation which is matrix-matrix multiplication. At compile-time, MatRox extracts structure information with modulerizerd compression.  The node blocking and coarsening algorithms are used to analyze this structure and to lower an internal representation of the evaluation operation. Structure analysis also leads to a efficient storage of the compressed data using a novel stroage format which we call CDS. The CDS stored generators and the generated evaluation code are used at runtime to compute the H-Matrix evaluation. 


%In MatRox the  to lower an internally generated evalatuion code .       MatRox modulerzies the compression phase in H-Matrix appoxiamtions, as a result, it is able to  and a  for generating highly efficient code for the evaluation phase of H-matrices. MatRox looks into the structure of a matrix and generates an efficient code for the given structure by decoupling structure analysis from the evaluation phase. The input code to MatRox is shown in \autoref{fig:input} where it takes the admissibility condition (parameter $\tau$ in Equation\ref{eq:ad}), the point set, the kernel function, and sub-block accuracy requirement as inputs and generates an efficient evaluation code and a compressed matrix stored in a format called the compressed data-sparse storage (CDS) format. The generated code, i.e., the evaluation phase, will be compiled and ran using CDS as its input.
 %To deal with the scenarios that the user needs to change the kernel function or tune accuracy, MatRox also has another solution in which compression is moved to run-time to reuse part of structure information. we will discuss about it in ~\autoref{sec:matroxrc}.
 %MatRox has two major components: Structure extraction \& analysis (Struct-EA) and a code lowering pipeline. Struct-EA first extracts the structure information which includes: \textit{(i)} the cluster tree, \textit{(ii)} the near-far interaction list, \textit{(iii)} the sampling-based nearest-neighbour list, and \textit{(iv)} the rank information with generators.  The generated structure information is then analyzed in Struct-EA to create \textit{structure sets} and the CDS-stored H-matrix.  The code lowering phase uses the structure sets to transform the evaluation code. In this section we go over all these components. 

\begin{figure}
    % \hspace{1cm}
    \centering
    \input{Figures/inputcode.tex}
    \centering
    % \subfloat[]{\Input{F}}
    % \includegraphics[width=0.75\columnwidth]{\Input{Figures/inputcode.tex}}

    \caption{MatRox input code}
    \label{fig:input}
\end{figure}

%\subsection{Evaluation} \textcolor{blue}{I think we need a section here to talk about evaluation before we start analysis and lowering. Otherwise it is covered in ME well.}

\subsection{Modulerizing Compression}\label{sec:sa}
%\autoref{fig:structure} shows an overall view of the struct-EA component of MatRox. As shown, structure extraction takes the admissibility condition, point set, kernel function, and the accuracy requirement as inputs. It then constructs the cluster tree and  computes interactions based on the admissibility condition followed by sampling and low-rank approximation that generate the approximated sub-blocks of the H-matrix. These four components are jointly referred to as the compression phase in existing libraries however, MatRox decomposes the compression phase into four components to be able to reuse information whenever possible. We explain how MatRox reuses the output of compression in Section 4.  

\begin{figure*}
    \centering
    \includegraphics[width=2.0\columnwidth]{Figures/matrox-sa.jpg}
    \caption{Structure extraction \& analysis (Struct-EA)  phase in MatRox}
    \label{fig:structure}
\end{figure*}


\begin{figure}
    \centering
    \input{Figures/matroxrun.tex}
    \caption{MatRox runtime code}
    \label{fig:matroxrun}
\end{figure}

We separate different components of compression to extract three structure information  that will guide the analysis stage. The 


\textbf{The cluster tree.}
As shown in \autoref{fig:structure}, the input to the tree construction component is the point set and it constructs the cluster tree as output. Points are partitioned using tree structure, in which root node is assigned the full set of points and the tree is built recursively by partitioning the points corresponding to each node and assign it to the children of the node. The partitioning continues until the number of points in the current node is less than a pre-defined constant $m$ named \textit{leaf size}. 
In MatRox, we use kd-tree \cite{omohundro1989five} for low-dimensional points (1-3d). kd-trees are class of partitioning that does partitioning along the coordinate dimension of maximum spread.
When the number of dimensions go beyond three, kd-tree methods are not efficient because it performs partitioning along one dimension ~\cite{rajani2015parallel}. Thus for dimensions more than three MatRox uses recursive two-means ~\cite{rebrova2018study} which is a special variant of k-means for high dimensional points. k-means methods perform partitioning based on geometry distance between points and is shown to be efficient in existing high dimensional point \cite{dasgupta2008hardness}. As you can see the shape of tree is determined by the partitioning and partitioning depends on the point distribution. For example, if points are distributed uniformly, such as points in \autoref{fig:point}, the resulting tree will be a perfect binary tree, otherwise it will be a imperfect binary tree.
%Therefore, the output of tree construction is a binary tree, which we refer to as \textit{cluster tree}. 

% partitions the point set hierarchically and represents the hierarchy using cluster tree.  The root node is first
% Cluster tree provides block size information as well as the dependency between blocks. For example in \autoref{fig:motivation}, every node of the cluster tree represents a partition in the point set and each edge shows a dependency between two blocks.


%TODO the tree is a general binary tree which could be balanced as shown in ?? or can be ombalanced. Why is this? What property of point set will be revelead by having this? 
%TODO make sure to indicate this wherever this generality increase complexity e.g., in tree coarsening

\textbf{The near-far interaction list. } 
As shown in ~\autoref{fig:structure}, the input to the interaction computation component is cluster tree and admissibility condition and it produces near and far node lists as outputs. Since each node of the cluster tree is assigned to a set of points, we can find low-rank blocks by quantifying the interactions between tree nodes based on admissibility condition shown in Equation \ref{eq:ad}.  
Figure \ref{fig:weak} which shows a weak admissibility condition, $\tau$ is $\infty$, near interactions are $\{(3,3),(4,4),(5,5),(6,6)\}$ and far interactions are $\{(1,2),(2,1),(3,4),(4,3),(5,6),(6,5)\}$. %, in which all off-diagonal blocks are low-rank shown in Figure \ref{fig:hss}. 
%Figure \ref{fig:strong} shows the strong admissibility condition in which $\tau$ is set to allow that interactions between different nodes can not satisfy the condition. In other words, some of the off-diagonal blocks are full-rank. 
%In this case, near interactions are $\{(3,3),(3,4),(4,3),(4,4),(5,5),(6,6)\}$ and far interactions are $\{(1,2),(2,1),(5,6),(6,5)\}$, in which the matrix structure is shown in Figure \ref{fig:h2}. 
%Therefore, the output of interaction computation is near and far interaction list mentioned above. 

%After tree construction and interaction computation, most structure information is known except the rank. The exact rank information is only known after the compression phase. 
% takes point set and admissibility condition as input and measures the interaction between different parts of point set and decide what interactions are far and what interactions are near. The equation for deciding about far or near interaction is shown in~\ref{eq:ad}. 
% For example, Figure \autoref{fig:weak} and ~\autoref{fig:strong} show weak and strong admissibility respectively, which results in different matrix structures shown in Figure \ref{fig:hss} and \ref{fig:h2}. 

\textbf{The nearest neighbor list from sampling.}
 The input to the sampling phase is the point set and the cluster tree, the output is a nearest-neighbor list for each sub-domain which is used to reduce the complexity of the low-rank approximation phase. "The low-rank matrices U,V can be either analytically computed using expansions of the kernel function, or semi-algebraically computed using fictitious points (or equivalent points), or using algebraic sampling-based
methods that use geometric information []." Matrox uses the later approach. The sampling phase creates a list that guides the sampling based low-rank approximation. The point set is used to construct the  k-nearest-neighbour list of each point. The cluster tree is then used to merge the nearest-neighbour list of points in the same sub-domain. Neighbor-based importance sampling~\cite{march2015askit} is then used to sample from this  nearest-neighbour list.

%MatRox performs low-rank approximation on off-diagonal blocks using interpolative decomposition (ID) which is computed by rank-revealing and pivoted QR factorization. 
%To reduce the ID overhead, we approximate ID by subsampling the rows of off-diagonal block, which is related to sampling nearest points for each point.
%MatRox uses neighbor-based importance sampling~\cite{march2015askit} to create the nearest-neighbors of each sub-domain using a greedy search excluding neighbours within the same sub-domain. the sub-domain used in nearest neighbor search is different from  the cluster tree


% performs an approximation based on capturing the row space of a matrix block that eventually leads to an efficient compression phase. 
\textbf{Rank information and the generators.} 
The inputs to the low rank approximation block in MatRox is the cluster tree, the kernel function, the sampling information, and the accuracy requirement and the outputs are the ranks of the approximated sub-blocks as well as their U, V, B generators.
The off-diagonal blocks $K_{v_1,v_2}$ corresponding to the interaction between node $v_1$ and $v_2$ can be approximated as 
\begin{equation}\label{eq:off}
K_{v_1,v2} \approx \widehat{U}_{v_1} B_{v_1,v_2} (\widehat{V}_{v_2})^{T}
\end{equation}
where  $\widehat{U}_{v_1}$ is a tall-skinny matrix and $\widehat{V}_{v_2}^T$ is the transpose of bases for the column and row spaces of $K_{v_1,v_2}$. 
The bases  $\widehat{U}_{v_1}$ and $\widehat{V}_{v_2}$ are not stored explicitly since they are constructed hierarchically from their children.  
For an internal node $\eta$ with children $c_1$ and $c_2$,  $\widehat{U}_{\eta}$ and $\widehat{V}_{\eta}$ are defined as
\begin{equation} \label{eq:nested}
\widehat{U}_{\eta} = \begin{bmatrix}
\widehat{U}_{c_1}  & 0 \\
  0  & \widehat{U}_{c_2}
\end{bmatrix} U_{\eta}
\textrm{   and   } 
\widehat{V}_{\eta} = \begin{bmatrix}
\widehat{V}_{c_1}  & 0 \\
0  & \widehat{V}_{c_2}
\end{bmatrix} V_{\eta}
\end{equation}
Except for leaf nodes that $U_\eta$ and $V_\eta$ are stored on node $\eta$ because $\widehat{U}_{\eta} =U_{\eta}$ and $\widehat{V}_{\eta}=V_{\eta}$, for the remaining nodes, ${U}_{c_2}$, ${U}_{c_2}$, ${V}_{c_1}$, and ${V}_{c_2}$ are stored as shown in \autoref{eq:nested}. 
MatRox approximates low-rank blocks using interpolative decomposition (ID) \cite{cheng2005compression} to compute the nested bases $U$ and $V$, i.e. the generators, in Equation \ref{eq:off} along the tree, in which sampling information is used to reduce the overhead.The  Kernel function is used to compute the subsampled matrix block on the fly and the accuracy requirement is used to determine the rank with which we approximate a matrix block; we use adaptive approximation  similar to []. 
% Here, interaction information is not required since $U$ and $V$ can be generated along the tree without knowing interaction information. 
The output of this stage is $U$, $B$, $V$ generators to approximate original matrix as well as rank information. 

% takes sampling information and the cluster tree in addition to kernel function and accuracy requirement and computes the low-rank representation for each block of the matrix. 

\subsection{Structure Analysis}\label{sec:sa}
After finishing compression, all structure information are known and MatRox analyzes this information in the node blocking and coarsening phases to create structure sets that will be used later for code generation. The low-rank blocks  along with structure analysis information are used for building CDS in the data layout construction block.

\textbf{Node blocking.} As shown in \autoref{fig:structure}, the node blocking component inspects interaction computation information as well as tree information to generate block set for improving locality in far and near nodes. The generated blockset will be later used for transforming the code in Section \ref{sec:codelowering}.  
Algorithm ~\autoref{alg:nodeblock} shows how MatRox constructs \textit{fblockset} for far interactions. % The block set on near interaction can be generated using the same idea. 
Assuming the number of nodes except root node is N. 
In line \ref{line:bnblk}-\ref{line:snblk},  the node blocking algorithm goes over 
$N \times N$ possible interactions and maps valid interactions in \textit{far} set into
\texttt{blocks} grid with size of $N/blockSize \times N/blockSize$ based on the index of nodes involved. 
In line \ref{line:bset}-\ref{line:sbset}, MatRox inspects the non-empty cells of \texttt{blocks} and gather them into \texttt{fblockset}.
%The block set is used to perform code transformation, which exploits the locality existing in interactions and generate efficient code to perform the computation related to interaction part. 
We take Figure \ref{fig:strong} as an example to illustrate \autoref{alg:nodeblock}. The input \textit{far} interaction list to Algorithm ~\autoref{alg:nodeblock} is $\{(1,2),(2,1),(5,6),(6,5)\}$ and \textit{blocksize} is 2. After first stage shown by line 2-8, {blocks[0][0]} includes far interactions $\{(1,2),(2,1)\}$ and {blocks[2][2]} includes far interactions $\{(5,6),(6,5)\}$. 
After second stage shown by line 9-16, blocks[0][0] is added to fblockset[0], fblockset[1] is empty and block[2][2] is added to fblockset[2] and final fblockset is $\{\{(1,2),(2,1)\}; \{(5,6),(6,5)\};\}$. 
 
interactions will eventually update a part of y vector and since several interation might need to access to the same location of y, synchronization is required.
Node blocking ensures that interactions that are writing to the same part of y are run in the same thread. 


% block interactions between nodes in order to improve locality. 
% \autoref{alg:nodeblock} show how MatRox inspects the cluster tree and interaction information to build block set i.e., \texttt{fblockset}. 
%
\begin{algorithm} [!ht]
\caption{HTree node blocking for far nodes}	\label{alg:nodeblock}
	\SetAlgoLined
%	\begin{small}
				\SetKwInOut{Algorithm}{Algorithm}
			\SetKwInOut{Input}{Input}
			\SetKwInOut{Output}{Output}
			\Input{$HTree$, blockSize}
			\Output{fblockset}
% 			\If{NorF == far}{
% 			    blockDim = (Tree.numNodes - 1 + blockSize) / blockSize
% 			}
% 			\Else{
% 			    blockDim = (Tree.numLeafNodes - 1 + blockSize) / blockSize    
% 			}
			$blockDim$ = (HTree.numNodes - 1 + blockSize) / blockSize \\
			blocks[$blockDim$,$blockDim$] = {(0,0)}; \\
			\tcc{Find blocks based on far interactions}
			\For{every node x $\in$ HTree and x != root }{ \label{line:bnblk}
			    idx = (x-1) / blockSize \\
			    \For{node y $\in$ HTree.far[x]}{
		        idy = (y-1) / blockSize \\
			    blocks(idx,idy).append(x,y)    
			    }
			}  \label{line:snblk}
			
			\tcc{Add blocks into fblockset }
			\For{i=0; i<blockDim; i++}{ \label{line:bset}
			    \For{j=0; j<blockDim; j++}{
			        \If{
			        blocks(i,j).size() > 0 }{
			          fblockset[i].append(blocks(i,j))  
			        }
			    }
			}\label{line:sbset}
%	\end{small}
\end{algorithm}

\textbf{Tree coarsening.} As shown in \autoref{fig:structure}, tree coarsening inspects the structure information obtained from the cluster tree and also rank information of compressed blocks and find a static scheduling that provides a load-balanced parallel implementation. There are two kinds of irregularity that affects the efficiency of the evaluation phase: the irregular dependency coming from the cluster tree and different computation cost for each node of the cluster tree due to different rank. MatRox aims for scheduling tree nodes on a parallel shared memory architecture that preserves locality and provide a load-balanced implementation. To solve this issue we adopt an existing solution called load-balanced level coarsening (LBC)~\cite{cheshmi2018parsy} which is proposed for sparse matrices and ensures locality and load-balanced in a parallel implementation.   
%the   MatRox applies the revised Load-Balanced Level Coarsening (LBC) [*ref*] specific to the tree with rank information to generate coarsen level sets.
%Since the hierarchical matrix computation is performed through tree traversal, tree can be treated as a dependency graph and rank information can be used to estimate the cost of computation on each node.  

As shown in Algorithm \ref{alg:partAlg}, the inputs to tree coarsening algorithm is the cluster tree $CTree$, rank information $rank$, the number of requested partitions $k$, and one tuning parameter $agg$ that define how coarse each partition will be after coarsening. The output of this component is coarsened set that will be used in code lowering phase in Section \ref{sec:codelowering}. 
The algorithm proceeds in three stages: 1) compute the cost of computation on each node based on rank information shown in line \ref{line:bcost}-\ref{line:ecost}. As shown, the cost of a leaf node is computed different than other nodes.  2) find disjoint sub-trees for each coarsen level shown in line \ref{line:bcoarsen}-\ref{line:ecoarsen}. \textit{Tree[lb:ub]} represents a subtree of $Tree$ that includes levels in range of lb-ub. Subtrees in \textit{Tree[lb:ub]} is stored in postorder to preserve temporal locality between parent and children nodes.  3)merge the sub-trees such that the cost of each merged partition is balanced shown in line \ref{line:bpack}-\ref{line:epack}. Binpacking algorithm in line \ref{line:binpack} uses rank information to create balanced partitions using a variant of the first-fit decreasing bin packing approach similar to \cite{coffman1978application}. 
%In the second stage, we keep each disjoint sub-tree in postorder to enable data reuse from children nodes to parent node. 
%The algorithm assumes topologically-order level set is generated starting from leaf node coupled with the tree. 
%The output of tree coarsening is coarsen level set, which enables code transformation, which exploits parallelism from tree in a static manner and also guarantees locality and load balance.


% generate level sets; 2) merge every $agg$ level sets; 3) merge sub-trees in each coarsen level.  
% % Line \ref{alg:level}-11 of Algorithm \ref{alg:partAlg} creates topologically-ordered level set starting from leaf nodes, in which parent(x).nd, the nd property means the number of dependencies from children nodes and its value is 2 and 0 for non-leaf and leaf node respectively.  In line 13-19, the algorithm \ref{alg:partAlg} groups every $agg$ levels into one coarsen level and find disjoint sub-trees by performing post-order traversal. Then, the sub-trees are kept in post-order to promote locality.  In line 27-32, a bin packing algorithm is used to merge sub-trees into $nPart$ partitions with balance cost.  
% Coarsen level set is used


%TODO: put rank information as input
%TODO: use label for line numbers, this is hard to maintain.
\begin{algorithm}
		\caption{Cluster tree coarsening }
		\SetAlgoLined
	%	\begin{small}
			\label{alg:partAlg}
			\SetKwInOut{Algorithm}{Algorithm}
			\SetKwInOut{Input}{Input}
			\SetKwInOut{Output}{Output}
			
			%\underline{LBC Algorithm} \;
			%\Algorithm{\LBCfull{}}
			\Input{$CTree, k, agg, rank$}
			\Output{CoarsenSet}
			%Generate a topologoically-ordered level set 
			%$levelset$ = build\_level\_set($Tree$)\\
% 			\tcc{Generate level sets from tree}
% 			\For{node $x \in $ Tree.leafnodes}{
% 				levelset[$Tree.depth$].append($x$)
% 			}
% 		%	\tcc{Generate level sets for non-leaf nodes}
% % 			\For{l=Tree.depth-1; l=1; l--}
% % 			{
% % 				\For{node $x \in $ levelset[l+1]}{
% % %					\tcc{Decrease dependencies of parent node} 
% % 					$--$$(parent(x).nd)$ \\
% % %					\tcc{Add node $x$ in levelset if its children nodes have been processed}
% % 					\If{(parent(x)$.$nd)==0}{
% % 						levelset[l].append(*(x.p))
% % 					}		
% % 			    }				
% % 			}
			%\tcc{Generate coarsen level sets}
% 			idx = 0 \\
% 			\For{l=Tree.depth-agg+1; l$>=$1; l-=agg}{ \label{alg:level}
% 			    %ST = post\_order($Tree[l:l+agg]$);\\
% 			    CoarsenSet[idx].append($Tree[l:l+agg]$);\\
% 			    ++idx;\\
% 			}
% 			\For{l=Tree.depth-agg+1; l$>=$1; l-=agg}{ \label{alg:level}
% 									\tcc{Find subtrees between level l and l+agg}
									
									
% 				\For{node $x \in$ levelset[l]}
% 				{
% 				%	sT.root = $\&$x \\
% 					ST=Postorder(levelset, x, l, l+agg) \\
% 					CoarsenSet[idx].append(ST)
% 				}
% 				++idx
% 			}
			
% 			Cost estimation for each node based on rank information \\
			$l = \lceil CTree.height / agg \rceil$ \\
			\For{ i=0; i<$l$; i++}{\label{line:bcoarsen}
	    		lb = i*agg; \\
				ub = (i+1)*agg; \\
			    \tcc{Find disjoint subtrees}	
				cl = disjoint\_subtrees(CTree[lb:ub]); \\
			    CoarsenSet.append(cl);
			}       \label{line:ecoarsen}
			
			
			
			\tcc{Cost estimation for each node}
			\For{ node $ x \in CTree$}{\label{line:bcost}
				\uIf{ x $\in$ CTree.leafnodes}{
%					\tcc{leaf node}
					CTree[x].cost = cost(rank(x)) \\
				}
				\Else{
					\tcc{Non-leaf nodes require rank information from children}
					CTree[x].cost = cost(rank(x), rank(lchild(x))+rank(rchild(x)))
				}	
			} \label{line:ecost}
			\tcc{Merge subtrees in each coarsen level}
			\For{i=0; i<$l$; i++ }{\label{line:bpack}
			    cl = CoarsenSet[i] \\
			    nPart = cl.size() $>$ k ? k : cl.size()/2 \\
			    CoarsenSet[i] = bin\_pack(cl, nPart); \label{line:binpack}
			} \label{line:epack}
			
% 			\For{ i =0; i<$l$; i++}
% 			{
% 				\tcc{Merge subtrees in each coarsen level}
% 					nPart = cc $>$ k ? k : cc / 2; \\
% 					cl = bin\_pack(Tree[lb:ub], nPart); \\
% 					CoarsenSet.append(cl);
% 			}
			
% 			\For{ cl $\in$ {CoarsenLevelSet}}
% 			{
% 				\tcc{Merge subtrees in each coarsen level}
% 				\If{cl.size() $>$ 1}{
% 					nPart = cl.size() $>$ k ? k : cl.size()/2 \\
% 					cl = BinPack(cl, nPart);
% 				}
% 			}	
	%	\end{small}
\end{algorithm}


\begin{figure}
    \centering
    \subfloat[CDS for HSS]{
    \includegraphics[width=0.5\columnwidth]{Figures/hsssf.pdf}
    \label{fig:cdshss}
    }
    \subfloat[CDS for H2]{
    \includegraphics[width=0.5\columnwidth]{Figures/fmmsf.pdf}
    \label{fig:cdsh2}
    }
    \caption{The compressed data-sparse format (CDS) for hierarchical matrix, we do not show the V generators for space.}
    \label{fig:cds}
\end{figure}
%TODO: draw CDS in general form, and in the side show two examples for the motivation example. 
\textbf{Data layout construction.} As illustrated in \autoref{fig:structure}, the data layout construction component stores the low-rank blocks of the low-rank approximation component into a new storage format, called compressed data-sparse storage (CDS), based on the computation pattern that is decided in node blocking and tree coarsening components. Since CDS considers the order of computation, which is mainly depends on the structure, it improves the locality of computation in the evaluation phase. 

%TODO: we might need one paragraph here to describe two different nature of the evaluation phase and the talk about why storage format improves locality. should be able to copy from Arxiv paper.

Figure~\ref{fig:cds} shows how different low-rank blocks of matrices in the ~\autoref{fig:motivation} are stored in CDS format. As shown, CDS has three major parts that store different full-rank blocks $D$ from originla matrix, and the generators $B$ and $U$ consecutively in arrays \texttt{Dgen}, \texttt{Bgen}, and \texttt{Ugen} respectively. Since the low-rank blocks are stored in compressed way, \texttt{Dptr}, \texttt{Bptr}, and \texttt{Uptr} point to the starting point of a block in the \texttt{D}, \texttt{B}, and \text{U} arrays. 
The order of storing matrix blocks is based on computational order to improve spatial locality guided by structure-specific transformation. For example,
as shown in \autoref{fig:cds}, the effect of block transformation is visible in \texttt{Dgen} where $D_{3,3}$, $D_{3,4}$, $D_{4,3}$ and $D_{4,4}$ are stored in order based on blocking to improve the locality. 
Since computations related to $U$ are performed through tree traversal, therefore, the order of storing $U$ is also based on the order of accessing tree nodes during tree traversal. 


% the order of ?? and ?? are changed to improve locality. 

\subsection{Code lowering}\label{sec:codelowering}
Code lowering part of MatRox uses information of the structure analysis through structure sets and generate a code for the given sets. \autoref{fig:lowering} shows a general overview of the code lowering part. As shown it starts with an initial AST that is internally represents the evaluation phase, i.e., matrix-vector multiplication  using the MatRox intermediate representation. Then MatRox applies either or both transformations internally based on structure sets. Further low-level transformation that can be hinted by the analysis is done afterwards and then the optimized C code is generated. In this section we explain the details of each transformation block in the code lowering part of MatRox. %Matrox uses Sympiler~\cite{} for intermediate representation.  

\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/codelowering.jpg}
    \caption{MatRox with the details of code lowering pipeline}
    \label{fig:lowering}
\end{figure*}

\textbf{Block transformation}
enables the generated code to benefit from the locality for interaction-based computation in the evaluation phase by using the give block-set. 
The general form of blocking transformation is shown in Figure \ref{fig:transformation} (c) and (d). 
The loop is annotated with keyword \texttt{block} which shows the block inspector-guided transformation can be applied. For example,
for HSS-structure matrix shown in Figure \ref{fig:weak} and \ref{fig:hss}, the blocking transformation will not be activated because the interaction-based computation is performed on diagonal blocks and blocking strategies will not improve the locality.
For general H2 matrix, if the number of blocks is larger than a threshold, the MatRox will apply block transformation. 
The threshold is a constant number that is tuned for each architecture to provide performance benfits. 
% aggregates  computation from both far and near interactions to improve locality. 


% \begin{figure*}
% \centering
% \begin{tabular}{c c}
%   \subfloat{  \input{Figures/level.tex}} \label{fig:level}
%   &  
%   \subfloat{\input{Figures/coarsen.tex}} \label{fig:coarsen}
%   %\input{Figures/coarsen.tex}
%   \\
%   	 {\footnotesize\textbf{(a) Before}} & {\footnotesize\textbf{(b) After}}\\
  
%      \hline
%     \subfloat{
%     \input{Figures/nonblock.tex}\label{fig:non-block}
%     }
%     \hspace{1.4cm}
%      & 
%      \subfloat{
%      \input{Figures/block.tex}\label{fig:block}
%      }
%      \\
%       {\footnotesize\textbf{(c) Before}} & {\footnotesize\textbf{(d) After}}\\
%       \hline
% \end{tabular}
% \caption{The inspector-guided transformations. Top: two nested loops in (a) are transformed into  loops over coarsen level set in (b). 
% Bottom: the two nested loops in (c) are transformed into loops over block set. 
% }
% \label{fig:transformation}
% \end{figure*}



\textbf{Coarsening transformation} enables the code to benefit from a balance between locality and load-balanced for far node computation of the evaluation phase by using the given coarsen-set. The general form of coarsening transformation is shown in Figure \ref{fig:transformation}(a) and (b). As shown the loop in Figure \ref{fig:transformation} (a) is annotated with keyword \texttt{coarse} that allows lowering phase to detect the loop that coarsening transformation is applicable to it. The transformed code is shown in Figure~\ref{fig:transformation} (b)  where the loops shown in lines \ref{line:bcl}-\ref{line:ecl} iterates over the given coarsen-set.


\textbf{Low level Transformations} further optimize the code by applying low-level transformation guided by structure information. Knowing the structure information such as, the cluster tree 
%and rank information 
allows application of some low-level transformation such as peeling. For example the last element of coarsen-set does not have tree parallelism thus, peeling its corresponding iteration and benefiting from block-level parallelism, e.g., using parallel BLAS is beneficial. 
% As another example when the rank of low-rank blocks are small, using a different BLAS routine that is optimized for small matrices will improve the performance. 

\textbf{Correctness check} At the beginning of the MatRox's generated code a light-weight checks are embedded to ensure the input data is consistent with the generated code. As discussed, two types of specialization happens in MatRox, specialization based on interaction when initial AST is generated and based on  H-tree structure in code specialization block. The specialization technique that is used in the current version of MatRox does not affect the correctness, it only affects the performance if the data is consistent with the code. However, the specialization based on interaction can result to a wrong output if the input data is not consistent. To avoid this situation, at the beginning of the MatRox-generated code and ensure the data/code combination is correct. There are two combinations that could result in wrong output, CDS for HSS with code for H2 and CDS for H2 with code for HSS. 
For the first case, if the interaction information integrated in block set shows it is HSS or no block set is provided, the flag about HSS will be true, the code will abort and require user to generate correct H2-based CDS . For the second case, if blockset is found from CDS, 
the code will recognize the input structure is H2, abort and require user to generate HSS-based CDS. 




%%%%% OLD material
% \begin{figure*}
% \subfloat[MatRox input code]{
% \includegraphics[width=0.75\columnwidth]{Figures/inputcode.pdf}
% }
% \hspace{0.5
% cm}
% \subfloat[Structure analysis]{
% \includegraphics[width=0.95\columnwidth]{Figures/matrox-sa.pdf}
% }
% \caption{The structure analysis phase in MatRox}
% \end{figure*}



%~\autoref{fig:overview} shows the overview of MatRox and how structure information is decoupled and used to perform structure-specific code generation. 
% Taking tree, kernel function and accuracy requirement as input, MatRox conducts compression phase that generates low-rank matrices to do approximation.
%Both approximation ranks and the low-rank matrices are known and included in the tree after compression phase.  Therefore, after extracting structure phase, all the structure information is known and passed to structure analysis phase, whose outputs are inspection sets including coarsen level sets and block sets. 
%The inspection sets are used for: 1) generate optimized code for evaluation; 2) guide the data layout transformation for efficient memory access. 



% [HERE we need to show the entire block diagram flow of MatRox A with the code in Solution A beside it]



% As shown in the figure, the user first inputs to matRox information of Kernel Function, the point set, accuracy and admissibility condition. The inputs are used to create structure information: (1) S1: create structure information that are extracted from the point set and the admissibility condition; (2) S2: conduct compression that generates the rank information. The structure information is then passed to the structure analysis phase. The outputs of the structure analysis which are the CDS storage format, the coarse set and blockset are the used to generate optimized code for evaluation. 




% For kernel matrices generated using kernel function and points, the structure from hierarchical matrix used to approximate kernel matrices is defined by four aspects: 
% \begin{itemize}
%     \item Tree information:  tree is built based on hierarchical partitioning of points to partition the matrix. Each tree node represents one cluster of points. 
%     Therefore, tree is determined only by points distribution. 
%     \item Interaction information: the interactions between tree nodes interpret the blocks in kernel matrix. 
%     Through quantifying the distance between two sets of points inside two tree nodes based on admissibility condition [*ref*], we define near and far interactions to perform low-rank approximation. 
%     If point sets in two nodes are away from each other, 
%     the interaction is defined as far interaction and the corresponding matrix block will be approximated; otherwise, it is near interaction and the corresponding matrix block will not be approximated.
%     The interaction information is determined by points distribution and admissibility condition.
%     % We use admissibility condition [] to quantify the interactions between two point sets in 
% \item Sampling information: To reduce the overhead of compression phase, neighbor-based importance sampling [*ref*] is used to capture the row space of matrix block and perform approximation. Since it is based on finding k nearest-neighbor points for each point, the sampling information only depends on points.
%     \item Rank information: it means that the approximation ranks for blocks associated with far interactions. Rank information is determined by points, kernel function and accuracy requirement. Rank information is known only after compression phase is done.    
% \end{itemize}


%MatRox optimizes the hierarchical matrix approximation problem by decoupling
%structure analysis due to the fact that most of structure information is only affected by points and will not change frequently. 

% By structure information we mean: and here is how they are obtained.
% Tree information → Only need points
% Interaction information → Only need points and admissibility condition
% Sampling information → Only need points
% Rank information → Only need accuracy requirement and kernel function and points



\section{Experimental Results}\label{sec:results}
We compare the inspector and executor performance of MatRox to the corresponding parts from STRUMPACK [], GOFMM [], and SMASH [], which are well-known libraries that provide Hmatrix approximation.  For data, we use eight machine learning datasets[] and five synthetic datasets.  The inspector performance for MatRox is quite similar to the existing libraries.  The resulting matrix-matrix multiply performed by the executor is much improved over existing library implementations due to improvements in data locality and parallelism.

\subsection{Methodology}
We select a set of datasets, i.e. points, shown in Table \ref{tab:dataset} from machine learning  and scientific applications. Problem IDs 1-8 are machine learning datasets from the UCI repository \cite{bache2013uci} and are high-dimensional points. Problem IDs 9-13 are scientific computing points that  are low-dimensional and are distributed along a curve or sphere \cite{cai2018smash}. The testbed architectures are shown in Table \ref{tb:platform}. All tools are compiled with  icc/icpc 18.0.1 using the \texttt{-O3} option. The median of 5 executions are reported for each experiment. 

We compare the performance of MatRox  to STRUMPACK \cite{ghysels2016efficient}, GOFMM \cite{yu2017geometry} and SMASH \cite{cai2018smash}, which are well-known libraries that implement $\mathcal{H}^2$ structures. %GOFMM supports two of the most commonly used  $\mathcal{H}^2$ structures FMM and HSS.
We use a binary cluster tree for all experiments with MatRox and the libraries.  
STRUMPACK only supports HSS, %We use FMM and HSS for comparisons to GOFMM, and use HSS when comparing to STRUMPACK. 
which is a specific class of  $\mathcal{H}^2$, with an admissibility condition  "large enough" (weak admissbility conidtion) \cite{hackbusch2015hierarchical} so that all off-diagonal blocks are low-rank approximated. In other classes of $\mathcal{H}^2$
the admissibility condition enables some off-diagonal blocks to also be full-rank , i.e. near blocks. In our experiment figures we use the keyword $\mathcal{H}^2$ for non-HSS structures.  The admissibly condition is  set  to a number larger than the diameter of the sub-domains ($\tau=100$ for all datasets) to create the HSS structure in MatRox.  GOFMM uses a \textit{budget} parameter, which operates differently from the admissibility condition, to create different structures. We implemented the algorithm used by budget in MatRox to compare to GOFMM. For HSS, budget is set to zero and for $\mathcal{H}^2$ it is  set to 0.03. SMASH takes as input only 1D-3D points and is primarily optimized for scientific kernels.  

%we also create the  to control the number of  low-rank blocks. , for instead of admissibility parameter. In GOFMM a budget of 0 creates the HSS structure. For FMM experiments, we set the budget to 0.03 in GOFMM and also implement the same budget algorithm in the MatRox internals so that we create the exact structure for fair comparison.

We use a Gaussian kernel \cite{williams1996gaussian} with bandwidth h = 5 when comparing to GOFMM and STRUMPACK; we use the machine learning datasets 1-8  for these experiments and dataset 9-13 are used as synthetic data for the Gaussian kernel. STRUMPACK does not run for all datasets; the random sampling used in their compression phase computes a matrix-matrix multiplication that does not fit in memory for large datasets. 
For comparisons to SMASH we use their default settings of kernel function $(1/\parallel x-y \parallel)$, the scientific pointsets ID 9-13, and the admissibility condition of 0.65; MatRox uses the same setting when compared to SMASH. 


%
%We use two most commonly used  $H^2$ structues called HSS and FMM are two of the commonly used $H^2$ structures that differ  on the number of low-rank approximated  off-diagonal blocks. In HSS all off diagonal blocks are low-rank approximated and only the diagonal blocks are full-rank, i.e. have near iteration, which FMM strucures have also ahve some off-diangoal blocks as full rank.  
%


%All libraries are installed and executed using the recommended default configuration. 
%In experiments related to SMASH, we use the kernel function $1/x-y$ similar to SMASH for MatRox.
%
 %When comparing MatRox to SMASH, we set the admissibility parameter to 0.65.
 
 
%and the libraries while it accepts different values based on a [FIXME: based on what?] for MatRox-RU experiments. 

%Structures such as HSS have only their diagonal blocks as full rank, i.e., near interactions, while some structures such as FMM also have off diagonals as full rank. As a result, the matrices with more off diagonal blocks that are full rank have less low rank approximated blocks. The admissibility parameter determines the number of low rank off diagonal blocks with smaller values leading to more low rank off diagonal blocks.

  %Problem 9 is a uniform $320 \times 320$ grid in $[0,1]^2$, problem 10 uses a random distribution of $65536$ points on a circle in 2 dimensions. Problem 11 and 12 are triceratops and sunflower geometry embedded in two and three dimensional domain from []. Problem 13 is the displacement of a set of $32000$ points on the unit circle from []. 
 

The \textit{sampling size} is $k=32$,  the \textit{leaf size} is $m=256$, the maximum rank in sranks is $256$, $agg$ is $2$,  \textit{blocksize} is $2$ for near and $4$ for far interactions, \textit{coarsen-threshold} is $4$, \textit{block-threshold} is equal to the number of leaf nodes. 
SMASH uses an adaptive method to determine the \textit{leaf size} which we also used in MatRox when comparing to SMASH. 
%internals so that we create the same structure to have a fair comparison. 
%We set the maximum rank in sranks to $256$ for all experiments. The $agg$ in coarsening block is set to $2$ and the \textit{blocksize} in node blocking is set to $2$ for near and $4$ for far interactions. \textit{coarsen-threshold} is set to $4$. \textit{block-threshold} is set to number of leaf nodes. 
%
The relative error that determines the overall accuracy of the HMatrix-matrix multiplication is 
$\epsilon_{f} = \lVert \widetilde{K}W - KW \rVert _{F} / \lVert KW \rVert_{F}, \textrm{for } W \in \mathbb{R}^{N\times Q}$
%
where $\lVert . \rVert_{F}$ is the Frobenius norm and $W$, which we refer to as the right-hand side (RHS),  is a randomly generated matrix with $Q$ the number of columns in $W$.
 $bacc$ is set to $1e-5$ for all experiments with MatRox and the libraries and the relative error is the same in MatRox and the libraries. 

%Structures such as HSS have only their diagonal blocks as full rank, i.e., near interactions, while some structures such as FMM also have off diagonals as full rank. As a result, the matrices with more off diagonal blocks that are full rank have less low rank approximated blocks. The admissibility parameter determines the number of low rank off diagonal blocks with smaller values leading to more low rank off diagonal blocks. Nonetheless, MatRox supports the generic  $\mathcal{H}^2$ matrices and can be used for different sparse structure matrices.

%The testbed architectures are shown in Table \ref{tb:platform}. All tools are compiled with  icc/icpc 18.0.1 using the \texttt{-O3} option. The median of 5 executions are reported for each experiment. 

\begin{table}[ht]
    \centering
        \caption{Experimental platform configurations [FIXME:fit to page]}
    \label{tb:platform}
    \begin{small}
    \begin{tabular}{|c| c| c|}
\hline
Processor         & \tabincell{c}{Intel \\ Xeon E5-2680 v3}   & \tabincell{c}{Intel \\ Xeon Phi 7250}  \\
  \hline
  Micro-architecture  &  Haswell  &  KNL\\
Frequency         &       2.5 GHz           &     1.4 GHz       \\
Physical cores    &         12              &     68             \\
Last-level cache  &         30 MB           &     34 MB            \\
\hline
Peak DP performance &       480 Gflops              &     3264.4 Gflops              \\
Peak memory bandwidth &     68 GB/s          &        115.2 GB/s             \\
\hline
    \end{tabular}
\end{small}
\end{table}


%with Id Matrices with ID 1-8 are generated from covtype,
%susy, and hepmass; covtype and susy are machine learning
% datasets. We use a Gaussian kernel [1] with bandwidth h = 10
% for these datasets. The kernel matrix form the points is of size N x N. 1-8 are machine learning datasets from UCI repository [*ref*] that have high dimensional points. Points 9-13 are scientific computing points that  are low dimensional point and are distributed along a curve or sphere. Problem 9 is a uniform $320 \times 320$ grid in $[0,1]^2$, problem 10 uses a random distribution of $65536$ points on a circle in 2 dimensions. Problem 11 and 12 are triceratops and sunflower geometry embedded in two and three dimensional domain from []. Problem 13 is the displacement of a set of $32000$ points on the unit circle from []. 
% We use a Gaussian kernel [1] with bandwidth h = 10
% for these datasets. 

%GOFMM  ,In this section, we compare the performance and scalability of the MatRox-generated code and MatRox-RU with state of the art libraries. We first explain the methodology and setup that is used for comparing with libraries, then we illustrate the performance MatRox-generated and MatRox-RU in comparison with state-of-the-art libraries. 

%We evaluate MatRox against three state-of-the-art libraries, namely GOFMM \cite{yu2017geometry}, STRUMPACK\cite{ghysels2016efficient} and SMASH \cite{cai2018smash} for hierarchical matrix computations. 



%In this section, we discuss the experimental setup and methodology.

%\textbf{Platform}
%The experiments are conducted on two architectures:
%Haswell (12-core, 2.5GHZ, Xeon E5-2680 v3) and KNL (68-core, 1.4GHz, Xeon Phi 7250). 
%All MatRox-generated code are compiled with  icc/icpc 18.0.1 using the -O3 option. 


%\textbf{Dataset}
%We selected a set of points from real applications listed in Table \ref{tab:dataset}.  Points with ID 1-8 are high dimensional machine learning datasets taken from the UCI repository [*ref*]. 
%Points with ID 9-13 are low dimensional points from scientific computing in which the point sets are distributed along certain curve or sphere. Problem 9 is a uniform $320 \times 320$ grid in $[0,1]^2$, problem 10 uses a random distribution of $65536$ points on a circle in 2 dimensions. 
%Problem 11 and 12 are triceratops and sunflower geometry embedded in two and three dimensional domain from []. 
%Problem 13 is the displacement of a set of $32000$ points on the unit circle from []. 

%TODO: many runs because 
%TODO: fig 11 compression
\begin{table}[]
    \centering
    \begin{small}
    \begin{tabular}{|m{6mm}|m{7mm} m{5mm} m{8mm} m{4mm} m{10mm} m{3mm} m{10mm}|}
%	\hline 
%Problem ID	& 1 & 2 & 3 & 4 & 5 & 6 & 7  \\ 
	\hline 
Name & covtype  & higgs & mnist & susy & letter & pen & hepmass \\ 
	\hline 
N	& 100k & 100k & 60k & 100k & 20k & 11k  & 100k  \\ 
	\hline 
d	& 54 & 28  & 780 &  18 & 16  & 16 & 28  \\ 
	\hline 
%Problem ID	& 8 & 9 & 10  &  11 & 12 & 13 &  \\ 
	\hline 
Name	& gas & grid  & random & dino  & sunflower  & unit &  \\ 
	\hline 
N	& 14k & 102k & 66k & 80k & 80k & 32k  &  \\ 
	\hline 
d	& 129 & 2 & 2 & 3 & 2 & 2 &  \\ 
	\hline 
\end{tabular} 
    \end{small}
    % \begin{tabular}{|c|c|c|c|}
    %      \hline
    % Problem ID     & Name & N & d \\
    %      \hline
    % 1    & covtype  & 100k & 54 \\
    % 2    & higgs & 100k &  28 \\
    % 3     & mnist & 60000 & 780 \\
    % 4     & susy & 100000 & 18 \\
    % 5     & letter & 20000 & 16 \\
    % 6    & pen &  10992 & 16  \\
    % 7     & hepmass & 100000 & 28  \\
    % 8     & gas    & 13910  &  129 \\
    % 9     & grid  & 102400   &  2 \\
    % 10     & random   &   65536  & 2   \\
    % 11     & dino        & 80000 & 3  \\
    % 12     & sunflower  & 80000 & 2\\
    % 13     & unit & 32000  & 2\\
    %      \hline
    % \end{tabular}
%     \begin{small}
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% 	\hline 
% Problem ID	& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 \\ 
% 	\hline 
% Name	& covtype & higgs & mnist  & susy  & letter & pen &  hepmass & gas  &  grid & random & dino  & sunflower  & unit  \\ 
% 	\hline 
% N	& 100k & 100k  & 60k & 100k & 11k & 100k & 14k  & 102k & 66k  & 80k & 80k &  & 32k \\ 

% d	& 54 & 28  & 780  & 18  & 16 & 16 & 28 & 129 & 2  & 2 & 3 &2  & 2 \\ 
% 	\hline 
% \end{tabular} 
%     \end{small}
    \caption{Data set: N is the number of points, d is the dimension of each point. }
    \label{tab:dataset}
\end{table}
%\textbf{Libraries}
%\textit{Structures:}
%Different H2 matrices have different structures. FMM and HSS are two examples of these different structures which are commonly used in applications. FMM is developed for N-body problem and integral equations frequently used in PDEs[*]. HSS methods are also used in kernel methods for statistical learning[]. 

% Structures such as HSS have only their diagonal blocks as full rank, i.e., near interactions, while some structures such as FMM also have off diagonals as full rank. As a result, the matrices with more off diagonal blocks that are full rank have less low rank approximated blocks. The admissibility parameter determines the number of low rank off diagonal blocks with smaller values leading to more low rank off diagonal blocks. Nonetheless, MatRox supports the generic  $\mathcal{H}^2$ matrices and can be used for different sparse structure matrices.


%\textit{Libraries:}We compare our results to the state-of-the-art libraries GOFMM, STRUMPACK, and SMASH. GOFMM supports both FMM and HSS and introduces a user-defiend parameter\textit{budget} that use point-disntances [] to control the number of off diagonal low rank blocks instead of admissibility parameter. STRUMPACK is a specialized library which only supports an HSS approximation
%of a square matrix (not necessarily SPD) and then uses it to construct
%an approximate factorization. SMASH is a unified library for general $\mathcal{H}^2$ matrix approximation, which is limited to 1-3 dimensional points due to the analytic techniques used in construction of $\mathcal{H}^2$ matrix.  All libraries are installed and executed using the recommended default configuration. 

% GOFMM does not control the number of off diagonal low rank blocks with admissibility, instead they use a parameter called budget that use point-disntances [] to determine the off diagonal blocks.

% In HSS only the diagonal blocks are full rank and all off diagonal blocks are low rank.

% In FMM besides the diagonal blocks that are full rank, some of the off diagonal blocks are also full rank.

% The admissibility condition determines the number of low rank off diagonal blocks. A smaller admissibility condition leads to more low rank off diagonal blocks, this is why in HSS the admissibility condition is set to infinity






% We evaluate the performance of MatRox by comparing to the state-of-the-art implementations of  low-rank approximation methods such as Fast Multiple Method (FMM) and HSS algoithms. 

% Furthermore, these methods have different structure assumptions  for approximating a SPD matrix. This makes HSS more efficient for approximating kernel matrices while ensuring a better load balance for FMM.







% We compare the performance of the MatRox to state-of-the-art libraries GOFMM, STRUMPACK, and SMASH. GOFMM implements algebraic Fast Multiple Method (FMM) and HSS low-rank formats. FMM is a rank-structured format that is similar to $\mathcal{H}^2$ with the difference that it supports more general shape of cluster tree~\cite{}.  [FIXME: the explanation of FMM and HSS are really messy here, we need a clean explanation that says why we think FMM and HSS are good cases of H2 to use for experiments. Discussions of the tree type are totally irrelevant to this paper, they seem to be written by someone that has not read the paper. ] 

% GOFMM uses a parameter called $budget$ to switch between HSS and FMM approximation, in which $budget$ controls the number of off-diagonal full-rank blocks.



% Since in this paper and also GOFMM, the cluster tree of FMM is limited to binary tree we use term $\mathcal{H}^2$ for the FMM implementation in GOFMM.  
% % STRUMPACK  is a specialized library for HSS approximation, which implements an HSS approximation of a dense matrix and uses it for an approximate factorization.

% SMASH is a library for geneal $\mathcal{H}^2$ matrix approximation, which is limited to 1-3 dimensional points due to the analytic techniques used in construction of $\mathcal{H}^2$ matrix.  
% All libraries are installed and executed using the recommended default configuration. 


%\textbf{Parameters setting}
%The inputs to MatRox and libraries are: points, kernel function (kfunc), admissibility parameter $\tau$ and the input accuracy $b-acc$. MatRox also has some internal parameters for inspector part which are explained in the following.

% \textit{Points:} 

%\textit{kernel function:} In all experiments related to GOFMM and STRUMPACK, we use the Gaussian kernel with with bandwidth $h=5$  for the libraries and for MatRox as well. In experiments related to SMASH, we use the kernel function $1/x-y$ similar to SMASH for MatRox.


%\textit{admissibility parameter and input accuracy:}For our HSS experiments, we set admissibility parameter to a number larger than the diameter of the partitioned point sets so that all off-diagonal are all low-rank  ($\tau=100$ for all datasets). In GOFMM a budget of 0 makes all off diagonal blocks as low rank which creates the HSS structure. For FMM experiments, we set the budget to 0.03 in GOFMM and also implement the same budget algorithm in the MatRox internals so that we create the exact structure for fair comparison. When comparing MatRox to SMASH, we set the admissibility parameter to 0.65. The input accuracy requirement $b-acc$ is set to $1E-5$ for all experiments in MatRox-generated code
%and the libraries while it accepts different values based on a [FIXME: based on what?] for MatRox-RU experiments. 




% [FIXME: is this really correct, also aren't we using different accuracies for MatRox-RU, if so, why are we suddenly generalizing to using ac a fixed value all over? Also there is no such thing as acc its $b_acc$]
% The input admissibility condition is set to $0.65$.  [FIXME: this is wrong you use different admisilbities all over.]

% The input accuracy requirement $acc$ is $1E-5$ to all libraries and MatRox if not specified.  [FIXME: Totally wrong, in MatRox-RU even the libraries are tested for differnet $b_acc$!]
% In compression phase, maximum possible rank for adaptive compression is $256$ and the number of nearest neighbours for each point in sampling part is set to 32 if not specified. [FIXME: use the key words introduced in italic in the moduler compression section, also is this for matrox and all libraries?] 


%When comparing to GOFMM and STRUMPACK in HSS case, the same binary perfect cluster tree is built [FIXME: why is the tree even relevant here]. The leaf node size is $256$.  [FIXME: use the key words introduced in italic in the moduler compression section, also is this for matrox and all libraries?] 
%When comparing to GOFMM in FMM case, the $budget$ is set to $3\%$, which means $3\%$ off-diagonal blocks will not be approximated. [FIXME: why? Is this still FMM, what made you make this choice? ] Other parameters and cluster tree are kept same as HSS case mentioned above [FIXME: very messy]
%For fairness, we take $budget$ as input to MatRox instead of the admissibility condition and use GOFMM's interaction computation method to identify off-diagonal full-rank blocks based on same cluster tree. [FIXME: what does fairnesss even mean?]



%[FIXME: first explain what SMash is, jstify why you are not using FMM and HSS in smash, tell them why you are using a specific admisiblity] Since SMASH builds cluster tree using kd-tree method and sets $\tau$ in admissibility condition to $0.65$ for problems in two or three dimensions, MatRox builds the same cluster and set $\tau$ to $0.65$ to guarantee the same HTree. MatRox keeps the same leaf node size as SMASH, in which leaf node size is determined based on admissibility condition and input accuracy requirement. [FIXME: what is the leaf node size, we cant just say its based on some random input] 


%As pointed in [], input accuracy requirement $b-acc$ reflects the error of the subsampled block [FIXME: these are now called submatricies] and may not correspond to the output error. This also occurs in GOFMM, STRUMPACK and SMASH. [FIXME: why are we suddenly bringing up the fact that the overall accuracy is not the same as int output accuracy! are we going to show a figure for this, very irrelevant, ]
%The number of columns in $W$ is $2048$ if not specified, and we will demonstrate the reason for the choice in next subsection. 
% in which .  
% When compared to GOFMM, the input admissibility condition $\tau$ to MatRox is used as $budget$ in GOFMM to keep fair comparison. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/hssnrhs.eps}
    \includegraphics[width=\columnwidth]{Figures/fmmnrhs.eps}
    \caption{ End-to-end comparison between MatRox and GOFMM, STRUMPACK for the number of columns in $W$ is $1$, $1024$, $2048$ and $4096$ for HSS (top) and $\mathcal{H}^2$-budget=0.03 (bottom) on Haswell.}
    \label{fig:nrhs}
\end{figure}


%\subsection{Performance of MatRox-Generated Code}


%In this section, we demonstrate that structure analysis strategies generate highly-optimized code coupled with CDS for hierarchical matrix computations compared to state-of-the-art libraries.

\subsection{Performance of the MatRox Inspector}

%
Figure \ref{fig:nrhs} shows the importance of improving the evaluation time with MatRox.   
%
% why compression are the same? the same algorithm, but it is large and using larger W col
%
The figure compares the MatRox  overall time, includes inspector and executor times, with  the overall time of libraries, i.e. compression and evaluation, for four  datasets and  RHS sizes if 1, 1K, 2K, and 4K on Haswell. The Matrox inspector time includes compression, structure analysis, code generation, and evaluation (executor).   While the compression time, for both $\mathcal{H}^2$-budget=0.03 and HSS and for all tools,  is a large fraction of the overall time for $Q=1$, for increasing $Q$ it will not change. The compression time of STRUMPACK is slower than MatRox and GOFMM because of using a different compression method. The cost of structure analysis and code generation of MatRox is also shown in Figure \ref{fig:nrhs} and is considerably smaller than the overall time. Structure analysis and code generation in MatRox is on average $8.1$ percentage of inspection time. 
Figure \ref{fig:nrhs} does not include SMASH because SMASH only supports matrix-vector multiplication ($Q=1$). We compared MatRox with SMASH for $Q=1$ and for datasets 9-10 our results show that the overall time of MatRox is on average 1.1$\times$ faster than SMASH and the evaluation in MatRox is 1.6 $\times$ faster than SMASH.

Figure \ref{fig:nrhs} shows that the evaluation time will becomes significantly larger with increasing $Q$ and thus performance benefits obtained from improving the evaluation time with MatRox will grow with $Q$. For example, for susy with $\mathcal{H}^2-budget=0.03$, MatRox's overall Speedup vs GOFMM is ** for $Q=1k$ and ** $Q=4K$.   %improvig the time for evaltuion using MatRox will In our experiments we select the size of $Q$=2k that is large enough to have an evaluation time close or larger than the compression time in most of dataset and thus amortized the compression time. % 
%This size is also reasonable for small datasets such as unit and grid where overall time of HMatrix-matrix multiplication is close to its equivalent dense matrix-matrix multiplication for $Q$ smaller than 2k.
\color{red}
In scientific computing applications such as multigrid methods, the coefficient matrix which comes from the discretization of elliptic PDEs \cite{gandham2014gpu} is multiplied by interpolation and restriction matrices \cite{briggs2000multigrid} which can have the same size


The Matrix-matrix multiplication is the main subroutines in scientific computing application such as multigrid methods where the fine grid coefficient matrix is multiplied by interpolation and restriction matrices \cite{briggs2000multigrid} in which the coeefiecnt matrix can have million of columns which come from the discretization of elliptic PDEs \cite{gandham2014gpu}. Similarly, Schur complement methods in hybrid linear solvers require dense matrix multiplications with millions of columns arising form PDEs \cite{yamazaki2010techniques}. high-order FEM schemes for hydrodynamics \cite{dong2014step}and direct-iterative preconditioned solvers \cite{im2004sparsity} are other examples that require large matrix matrix multiplications in their computations.

\color{black}


. We use a $Q=2K$ for the rest of our experiments unless stated otherwise.  
%
%
We also ran the un-approximated matrix-matrix multiplication $KW$ with GEMM and for the tested datasetes on average MatRox's overall time was 10$\times$ and 18$\times$ faster than GEMM for $Q=2K$ for HSS and $\mathcal{H}^2$-budget=0.03 respectively; the speedups obtained with HMatrix evaluation are significantly higher that GEMM for larger $Q$s.

%Figure \ref{fig:nrhs} shows the time MatRox speeds to do compression, structure analysis and code generation at inspection time. Figure \ref{fig:nrhs} shows the cost of structure analysis and code generation are small and is on average $8.1$ percentage of the entire inspection stage on Haswell.  Figure \ref{fig:nrhs} also shows the
%the accumulated time of MatRox, GOFMM and STRUMPACK using different number of right sides.
%As shown by Figure \ref{fig:nrhs}, when increasing number of right hand sides, the overhead from inspection including compression, structure analysis and code generation will be amortized and MatRox-generated code will provide more performance benefits.
%Since both GOFMM and MatRox are based on same compression algorithm, the time of MatRox in compression phase is almost as same as GOFMM.
%STRUMPACK is slower than other two tools because it uses matrix-vector product to perform random sampling in compression phase
% it requires a matrix times vector product for the random sampling phase in compression. [REPLACE THIS SENTENCE WITH SOMETING BETTER]
%Based on Figure \ref{fig:nrhs}, we set number of columns in $W$ to 2048 so that the performance benefits from MatRox-generated fast evaluation code  can be noticed.



\subsection{The performance the MatRox executor}
%role of each transformation
%role of data layout
% why letter is good, the number of near nodes?
%
%
Figure \ref{fig:sep} shows the performance breakdown of the MatRox's executor (evaluation) versus GOFMM and STRUMPACK for both HSS and $\mathcal{H}^2$-budget=0.03 on Haswell.   As shown MatRox's evaluation time is on average 3.41$\times$ and 2.98 $\times$ faster than GOFMM in order for HSS and $\mathcal{H}^2$-budget=0.03 and is on average 5.98$\times$ faster than STRUMPACK. The performance breakdown shows the effect of CDS as well as the block and coarsen algorithms. To show the effect of CDS, we run both the MatRox generated code, that uses CDS, and GOFMM and STRUMPACK, that use a tree-based storage format,  with a single-thread and label them in order with CDS (seq) and TB (seq). Coarsen, block, and low-level lowering applied to the MatRox code are labeled with in order coarsen, block, and low-level. The parallel version of GOFMM and STRUMPACK use a dynamic scheduling which are labeled with DS in Figure \ref{fig:sep}. 

%This subsection demonstrates how the combination of storage format CDS and structure analysis strategies outperform state-of-art libraries for hierarchical matrix computations.
%We show the performance of MatRox-generated code for both HSS and FMM case to demonstrate the effect of our proposed optimization techniques in different structures in Figure \ref{fig:sep}. 
%we run the MatRox generated code serially first to isolate the effect of CDS on performance comparing to tree-based storage used in libraries in Figure \ref{fig:sep}. 

Coarsening together with CDS  improves the performance of MatRox generated code  for both $\mathcal{H}^2$-budget=0.03 and HSS as shown in Figure \ref{fig:sep}.  CDS in MatRox improves the performance of the sequential code by improving locality on average $2.44\times$ and $2.20\times$ compared to sequential GOFMM for HSS and $\mathcal{H}^2$-budget=0.03. Coarsen lowering is applied to all matrices since the number of levels in all datasets are larger than \textit{coarsen-threshold}. 
Coarsening preserves locality and keep computation balanced in loops with carried dependencies and gives on average $79.2\%$ and $46.8\%$ performance improvement for HSS and $\mathcal{H}^2$-budget=0.03 respectively. 

In HSS, only the diagonal blocks have near iterations, the rest of the blocks are approximated as low rank which means their computations primarily involves loops with carried dependencies. Loops with carried dependencies dominate the execution time of the evaluation phase of HSS and thus coarsening shows a higher impact in HSS compared to $\mathcal{H}^2$-budget=0.03. Also, MatRox peels the last iteration of loops with carried dependencies to separately specialize  that iteration which  further optimizes loops with carried dependencies. This low-level transformation leads to on average $6.28\%$ and $4.24\%$ performance improvement of the MatRox code in order in HSS and $\mathcal{H}^2$-budget=0.03.  Since HSS is dominated by loops with carried dependencies, the effect of low-level transformation is also more prominent in HSS. 
  %
  %
Node blocking contributes on average $38.3\%$ to the performance of the MatRox generated code for $\mathcal{H}^2$-budget=0.03 on Haswell as illustrated in Figure \ref{fig:sep}. As shown, block lowering is not activated in HSS matrices because, the number of near interactions in HSS is smaller than the defined threshold in MatRox i.e., \textit{block-threshold}. 
%Since blocking applies to loops with reduction that involves interactions, the effect of blocking is higher in datasets with more interactions such as XX and XX that are improved XX and XX using blocking.    
  
  
One major goal of inspection and lowering in MatRox is to improve locality. Figure ~\ref{fig:loc} shows the correlation between the performance of the MatRox generated code versus the cost of average memory access among all datasets for both HSS and $\mathcal{H}^2$-budget=0.03 on Haswell.
%Figure \ref{fig:sep} shows the MatRox generated has different kinds of performance for different datasets. MatRox improves locality in all datasets but the level of improvement depends on properties of a dataset structure.  
We measured the average memory access~\cite{hennessy2011computer} in the evaluation phase of MatRox code and GOFMM using \texttt{PAPI} library by collecting L1, LLC(Last-level Cache), and TLB access and misses.  
The coefficient of determination or R2 is 0.81 that shows a close correlation between the improvement in average memory cycle and the achieved speedup. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/hss-separate.eps}
   \includegraphics[width=\columnwidth]{Figures/fmm-separate.eps}
    \caption{MatRox's generated code compared to GOFMM for HSS-structure approximation and $\mathcal{H}^2$-budget=0.03 approximation (bottom) on Haswell. seq denotes sequential, par denotes parallel, DS denotes dynamic scheduling, LL denots linked list. The effect of CDS, coarsening and low-level transformations are shown separately. [FIXME: Kazem wants you to change the legends, ask him.]
    }
    \label{fig:sep}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/local.png}
    \caption{The effect of locality on performance of the MatRox generated code. 
    }
    \label{fig:loc}
\end{figure}

  %The average improvement of MatRox-generated code over GOFMM and STRUMPACK is $3.41\times$ and $5.98\times$ in HSS, and  $2.98\times$ over GOFMM in FMM. 
%MatRox achieves $5.74\times$ speedup over GOFMM on the matrix generated from sunflower in HSS, in which the average \textit{srank} is 3. 
%The reason for the high speedup is when computation task related to $U$ and $V$ has low computation complexity on tree nodes, the execution time of computation on $U,V$ performed through tree traversal will be dominated by the memory access time on $U,V$ and MatRox-generated code can provide a better memory access on $U,V$ to reduce the execution time.  
  

%In HSS, no far interactions exist because the admissibility condition is 10,  and only the diagonal blocks have near iterations, the rest of the blocks are approximated as low rank which means they have to be computed with loops with carried dependencies.
%As shown by Figure \ref{fig:sep}, blocking is more effective in FMM case since HSS doesn't have enough interactions for node blocking,  because in HSS each leaf node is only near to itself while in FMM each leaf node can be near to other leaf nodes besides itself.
%The low-level transformation implemented in MatRox now is loop-peeling, which peels the last iterations of computations and exploit parallelism inside tree node during the computation is performance through tree traversal.
%Therefore, the low-level transformation is only applied to computations done through a bottom-up or top-down level-by-level traversal of the cluster tree.
%Low-level transformation leads to on average $6.28\%$ performance improvemnet in HSS  over $4.24\%$ performance improvement in  FMM case because computations performed through tree traversal take higher portion of time in HSS, FMM has more computations based on interactions than HSS because in FMM each leaf node has more near interaction nodes.
%  The average improvement of MatRox-generated code over GOFMM  is $2.98\times$. 
% , only diagonal blocks are kept full-rank and all off-diagonal blocks are approximated in low-rank, is simpler than FMM and requires less interaction information to represent the structure. 
% each node only has one far interaction node and each leaf node is only near to itself. 

% Since low-level 
% higher portion
% We show the benefits of MatRox-generated code by evaluating four factors separately, which are CDS, coarsening, blocking and low-level transformation shown in Figure \ref{fig:sep}. 
% To evaluate the effect of CDS separately, 
%  which peels last several iterations of nested computations because number of tree nodes in the single level is less than number of cores and parallelism inside tree nodes are exploited by using parallel BLAS.




% In the sequential configuration, the organization of data in CDS and computation is performed in the order as same as GOFMM computation order to show the effect of CDS. 

% In sequential setting, MatRox-generated code is faster than GOFMM and STRUMPACK by on average $2.44\times$ and $2.20\times$ on Haswell, %which benefits from the spatial locality provided by a continuous data layout in CDS. 
% Figure \ref{fig:sep} shows the performance of MatRox-generated code compared to GOFMM for HSS approximation, in which $budget=0$ enforces all off-diagonal blocks to be approximated in low-rank.
 %After coarsening and low-level transformation, the average improvement of MatRox-generated code over GOFMM and STRUMPACK is $3.41\times$ and $5.98\times$ on Haswell.  
%  MatRox achieves $5.74\times$ speedup over GOFMM on the matrix generated from sunflower with average rank $3$, which $2.11\times$ over GOFMM on the matrix generated from covtype with averge rank $225$. %The reason is GOFMM mainly focus on scheduling and exploiting parallelism from CTree and thus prefers computation-bound problem. The problem with low-rank structure is typically a memory-bound problem  and can benefits more from MatRox. 

 
% Figure \ref{fig:sep} also shows the performance of MatRox-generated code over GOFMM for FMM approximation.
% % , in which $budget=\%3$ enforces that $3\%$ off-diagonal blocks will not approximated based on geometry information from points. 
% The average improvement of MatRox-generated code over GOFMM library is $2.98\times$ on Haswell.In FMM approximation, the near and far interactions between tree nodes become irregular and blocking is applied to improve the locality. blockSize in Algorithm \ref{alg:nodeblock} for node blocking is tuned to 2 and 4 for near and far interactions respectively.  
% Figure \ref{fig:sep} shows that node blocking contributes on average $38.3\%$ of the overall performance on Haswell. % Since node blocking can be applied to both near and far interactions, the interactions can be blocked in either near or far block set. Node blocking may not provide significant performance benefits when there are not enough node blocks. For example, 
%dataset pen doesn't benefit from the node blocking strategies since few nodes are blocked.
% In HSS approximation, node blocking does not lead to performance improvement since each node is only far to it sibling node and each leaf node is only near to itself.
% Therefore, node blocking cannot block enough interactions to promote locality and provode performance benefits.

%Since SMASH uses a different algorithm for the compression phase, we compare MatRox code with SMASH in separate table shown in Table \ref{tab:smash}. 
%SMASH combines analytic technique (interpolation) with algebraic technique (rank-revealing QR decomposition) to construct low-rank blocks in compression phase.
%Due to the used analytic techniques, SMASH is limited to low-dimensional points.
%As shown by Table \ref{tab:smash}, SMASH's compression phase is faster than MatRox for 2-dimensional points due to the used analytic techniques with linear cost~\cite{}.  
%However, for 3-dimensional point dino, the compression in MatRox is $2.84\times$ faster than SMASH because the analytic techniques become extremely expensive with increasing dimension of points~\cite{}. Although the compression algorithm is different in SMASH and MatRox, the evaluation phase is similar. As shown in Table~\ref{tab:smash}, MatRox's evaluation phase is on average $1.70\times$ faster than SMASH. The relative accuracy 	$\epsilon_{f}$ is also reported in Table \ref{tab:smash} that is almost similar in all datasets. %even though the compression algorithm is different.  
% The objective of coarsening is promote data reuse between parent and children nodes and reduce the critical path of the tree by mergeing levels. 
% Especially, when the matrix is approximated in lower ranks, the hierarchical matrix computation becomes a memory-bound problem []. Therefore, the optimization techniques such as optimizing memory access and reducing the critical path of the parallel code can help while exploiting parallelism from the tree or increase number of cores does not help. 
% For example, for dataset sunflower in which the generated matrix with average rank 3 in off-diagonal blocks,  MatRox achieves $ 5.74 \times$ and $ 10.31\times$ over GOFMM. 
% The reason for higher speedup on KNL is also that MatRox utilize the memory bandwith more effectively. Low-level transformation in MatRox benefits from high-rank scenario, in which 
% the workload on each tree node in peeled tree levels is large enough to exploiting parallelism inside. 
% For example, for dataset mnist in which the generated matrix with average rank 227 in off-diagonal blocks,  low level transformation can bring $9\%$ performance improvement on KNL.
% % Figure \ref{fig:sephss} shows the effect of each factor  on the overall performance of MatRox-generated code. unit dataset doesn't benefit from low-level transformation on both Haswell and KNL, because the average rank of off-diagonal blocks is 2 and the workload is insufficient for parallelism.  
% We also notice that the low-level transformations provides more performance benfits on KNL because the number of cores increases to 68 and explioting parallelism inside tree nodes can bring more performance benefits when parallelism from tree is not enough. 

% From aspect of architecture, it requires the code to utilize the memory bandwidth effectively to harness the computation power of many-core processor KNL.


% The many-core processor KNL requires to utilize the memory bandwith effectively to harness the computation power 
 



% \begin{table}
% \begin{small}
% \begin{tabular}{|m{12mm}|m{4mm}m{6mm}m{4mm}m{4mm}c|m{4mm}m{6mm}c|}
% 	\hline
% \multirow{2}{*}{Dataset}	& \multicolumn{5}{|c|}{MatRox} & \multicolumn{3}{c|}{SMASH} \\
% \cline{2-9}
% 		& comp & sa & cg &eval
% 		 &$\epsilon_{f}$  & comp & eval & $\epsilon_{f}$  \\
% 	\hline
% grid	& 1.34 &0.03 & 0.01&0.08&9.32E-6 & 1.41& 0.15& 1.37E-6 \\
% random  & 0.54&0.01 & 0.01&0.03& 6.52E-6& 0.58& 0.04& 1.68E-6 \\
% dino  & 1.19&0.20 &0.01&0.32& 1.67E-6& 3.39& 0.59& 1.24E-6 \\
% sunflower & 0.68 &0.04 &0.01&0.04& 2.96E-6& 0.61& 0.05& 4.58E-6 \\
% unit & 0.39& 0.01& 0.01&0.03& 4.93E-6& 0.17& 0.06& 2.28E-6 \\
% \hline
% \end{tabular}
% \caption{The end-to-end comparison
% between MatRox and SMASH. 
% Numbers show the time in seconds. [FIXME: remove accuarcy]}
% \label{tab:smash}
% \end{small}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/fmm-separate.eps}
%     \includegraphics[width=\columnwidth]{Figures/knlfmmf.eps}
%     \caption{
%     MatRox's generated code compared to GOFMM for FMM-structure approximation on Haswell(top) and KNL(bottom). seq denotes sequential, par denotes parallel, DS denotes dynamic scheduling, LL denots linked list. The effect of CDS, coarsening and low-level transformations are shown separately.
%     % MatRox's generated code for evaluation phase compared to GOFMM for FMM-structure matrix. seq denotes sequential, par denotes parallel,  DS denotes dynamic scheduling, LL denots linked list.
%     }
%     \label{fig:sepfmm}
% \end{figure}
% \textbf{Overall performance}
% Since the compression phase is performed at compile-time in MatRox and its generated code for evaluation phase is performed at run-time. 
% Since MatRox takes compression to compile-time, generates optimized evaluation code by analyzing the structure and stores the generators in CDS order,  we 

% This section demonstrates the performance benefits provided by proposed structure analysis strategies and CDS over existing libraries.   
% \subsubsection{Overall performance in multiple runs}


% \textbf{Multiple runs}
% This section demonstrates MatRox-RU enables extra performance benefits in multiple runs by reusing the computations in the compression phase. 


\subsection{Scalability of the MatRox Executor}

Figure \ref{fig:scal} shows the scalability of the evaluation phase in MatRox vs. GOFMM, STRUMPACK, and SMASH for two different datasets on Haswell and KNL; other datasets follow a similar trend. SMASH does not support\textit{ covtype} and MatRox-Skernel is MatROx with SMASH settings.  
We selected KNL in addition to Haswell to demonstrate MatRox's strong scalability on a larger number of cores, i.e. 68 cores of KNL. MatRox scales well on both architectures while the libraries show poor scalability with increasing number of cores. For example, GOFMM's performance reduces from  34 to 68 cores in both datasets. MatRox's strong scaling is because coarsening and blocking improve improve locality and reduce synchronization while maintaining load-balance. %, that leads to a scalable evaluation code.    

%This section demonstrates better scaling in MatRox over state-of-the-art libraries. 
%Figure \ref{fig:scal} shows the scalability benefits of MatRox for different matrices and architectures. 
%While MatRox scales well on both architectures, GOFMM, STRUMPACK and SMASH are not scalable or scale weakly when number of core increases specically on KNL. 
%In Figure \ref{fig:scal}, we observe that  slow down in GOFMM from 34-core to 68-core on KNL. Although GOFMM uses the HTree as the input for dynamic task scheduling, the critical path from HTree is not reduced in GOFMM and the execution time of computations on the tree is bounded by task in the critical path of HTree, in which increasing the number of cores will not help. The tree coarsening used in MatRox will reduce the critical path by merging levels of HTree and also promotes the locality, thus MatRox shows better scalability. STRUMPACK doesn't scale well because it submits OpenMP tasks recursively along the tree and incurs the overhead of deep call stack in parallel code. Level-by-level traversal used by SMASH introduce unnecessary synchronization overhead and can not scale well. 

\begin{figure}
    \centering
    \includegraphics[width=0.45\columnwidth]{Figures/Mscalcovtype.eps}
    \includegraphics[width=0.45\columnwidth]{Figures/mscalunit.eps}
     \includegraphics[width=0.45\columnwidth]{Figures/mknlscalcovtype.eps}
    \includegraphics[width=0.45\columnwidth]{Figures/mknlscalunit.eps}
    \caption{Scalability result on Haswell (top two) and KNL (bottom two). Test Dataset: covtype (left) and unit (right).[FIXME: Increase fonts, makes colors different, increase the legend fonts. Replace linear scale with linear scaling, Replace Matrox-H2 with Matrox-Skernel, replace STRUMPACK with SUTRMPACK-HSS]}
    \label{fig:scal}
\end{figure}




% From figure \ref{fig:scal}, GOFMM scales better on covtype over unit while MatRox scales better on unit over covtype. The reason is related to structure of matrix, in which the matrix generated from covtype is with average \textit{srank} 225, computation complexity on $U,V$ in each tree node is high and exploiting parallelism from tree will help more,  and the matrix generated from unit is with average \textit{srank} 2, computation complexity on $U,V$ in each tree node is low and reducing memory access time will help more.





% GOFMM scales better on covtype than unit on both Haswell and KNL, while STRUMPACK scales better on unit then covtype on both Haswell on KNL. 



%The reason is also related to structure of matrix, in which the matrix generated from covtype is with averga rank 225 and the matrix generated from unit is with average rank 2. GOFMM prefers computation-bound problem (high-rank), which MatRox prefers memory-bound problem (low-rank). When switching from HSS to FMM and interactions between nodes become irregular, GOFMM scales better and MatRox scales worse shown by Figure \ref{fig:scal}. 

%GOFMM also adds interaction information to its run time scheduling system to schedule the tasks and therefore more parallelisms are exploited. In MatRox, node blocking is applied based interaction information, which priortizes locality over load balance. 
 %This is because the time of parallel code in GOFMM is bounded by critical path and increasing the number of core will not help. 
%STRUMPACK doesn't scale well because it submits OpenMP tasks recursively along the tree and  incurs the overhead of deep call stack. 
%Since SMASH only evaluations one right hand side, both MatRox and SMASH don't scale well due to insufficient computation task for parallelism. 
%Figure \ref{fig:scal} shows MatRox provides a scalable code by promoting locality. 

% don't gurantee load balance as coarsening, 

% GOFMM utilizes an out-of-order approach using dynamic scheduling to exploit the parallelism from both CTree and interaction information to schedule the task.   




